Mahler Measure for a Quiver Symphony

Adopting the Mahler measure from number theory, we introduce it to toric quiver gauge theories, and study some of its salient features and physical implications. We propose that the Mahler measure is a universal measure for the quiver, encoding its dynamics with the monotonic behaviour along a so-called Mahler flow including two special points at isoradial and tropical limits. Along the flow, the amoeba, from tropical geometry, provides geometric interpretations for the dynamics of the quiver. In the isoradial limit, the maximization of Mahler measure is shown to be equivalent to $a$-maximization. The Mahler measure and its derivative are closely related to the master space, leading to the property that the specular duals have the same functions as coefficients in their expansions, hinting the emergence of a free theory in the tropical limit. Moreover, they indicate the existence of phase transition. We also find that the Mahler measure should be invariant under Seiberg duality.

==> commented_out.tex <==
%================================================================
%Special cases for old choices for coeffs
Table \ref{Gammauni} classified in \cite{rodriguez2003hypergeometric}:
\begin{table}[h]
\centering
\begin{tabular}{c||c|c|c|c}
$\gamma$ & $[3]-3[1]$ & $[4]-[2]-2[1]$ & $2[2]-4[1]$ & $[6]-[3]-[2]-[1]$ \\ \hline
$a_1$ & $1/3$ & $1/4$ & $1/2$ & $1/6$ \\ \hline
$a_2$ & $2/3$ & $3/4$ & $1/2$ & $5/6$ \\ \hline
$\lambda_0^{-1}$ & 27 & 64 & 16 & 432 
\end{tabular}
\caption{}\label{Gammauni}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old choices for coeffs and properties
We list the Mahler measures as well as the periods for all 16 reflexive polygons in Appendix \ref{mahlerlist}. We find that there are four special classes which have particular simple forms (while it is not known whether the other cases could be written in a more compact form), and they are precisely the four special classes classified by Rodriguez Villegas \cite{rodriguez2003hypergeometric} as aforementioned. Moreover, as we shall discuss now, the dual polygons have the same $m(P)$ and $u_0(k)$ for these four classes \emph{only}, and in this sense we have 7 special polygons (3 dual pairs and 1 self-dual polygon).

In Table \ref{fourclasses}, we give the four special classes of reflexive polygons and their corresponding $\gamma$.
\begin{table}[h]
\centering
\begin{tabular}{c||c|c|c|c}
Polygons & 1 \& 16 & 2 \& 13 & 4 \& 15 & 7 \\ \hline
$\gamma$ & $[3]-3[1]$ & $[4]-[2]-2[1]$ & $2[2]-4[1]$ & $[6]-[3]-[2]-[1]$
\end{tabular}
\caption{The four special classes of polygons. From $\gamma$, one can read off the periods in terms of ${}_2F_1(a_1,a_2;1;\lambda_0^{-1}\lambda)$ from Table \ref{Gammauni}, where $\lambda$ denotes certain power of $k$ in each case.}\label{fourclasses}
\end{table}

As a result, the polygons in each class would have the same Mahler measure as well as period (and hence the condition for genus). As aforementioned, these polygons having the same Mahler measure are dual to each other. However, as one may check in Appendix \ref{mahlerlist}, for the remaining 9 polygons, the dual pairs have different Mahler measures and periods. It is easy to see the reason with the following theorem \cite{schinzel_2000,boyd2005small}.
\begin{theorem}
    Let $(0\neq)M=(M_{ij})_{n\times n}\in\textup{GL}(n,\mathbb{Z})$ and $\bm{z}=(z_1,\dots,z_n)$. Then $M(P(\bm{z}))=M(P(\pm\bm{z}^M))$, where $\bm{z}^M=\left(\prod\limits_{i=1}^nz_i^{M_{i1}},\dots,\prod\limits_{i=1}^nz_i^{M_{in}}\right)$. Hence, $m(P(\bm{z}))=m(P(\pm\bm{z}^M))$.
\end{theorem}
In other words, the Mahler measure for a Laurent polynomial with $n$ variables is GL$(n,\mathbb{Z})$ invariant. Hence, the four classes would have same Mahler measures respectively, where the transformation matrices are
\begin{equation}
    M_{16\mapsto1}=\begin{pmatrix}2&-1\\-1&2\end{pmatrix},~
    M_{13\mapsto2}=\begin{pmatrix}2&1\\0&1\end{pmatrix},~
    M_{15\mapsto4}=\begin{pmatrix}1&1\\1&-1\end{pmatrix},~
    M_{7\mapsto7}=\begin{pmatrix}1&0\\0&1\end{pmatrix}.
\end{equation}
However, the remaining 9 reflexive polygons are not related by any GL$(2,\mathbb{Z})$ transformation, even though there exists dual pairs. To show that there is no such transformation more explicitly, we can further use Pl\"ucker coordinates by virtue of its GL$(n,\mathbb{Z})$ invariance. In fact, by computing Pl\"ucker coordinates, we can quickly tell whether two polygons are related by GL$(2,\mathbb{Z})$ transformations. Let us start with a brief introduction to the notion of Pl\"ucker coordinates and quotient gradings.

The four special dual pairs which are actually related by quotient gradings while the remaining pairs are not. Pictorially, we draw the polygons No.16, No.13 and No.15 in black in Figure \ref{latticerefinement}. Then by quotient gradings, we mean that these polygons are transformed to some other polygons after certain refinement of the lattice (i.e., adding lattice points).
\begin{figure}[h]
    \centering
\tikzset{every picture/.style={line width=0.75pt}}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
%Shape: Grid [id:dp801478237910304] 
\draw  [draw opacity=0] (81,40.2) -- (121,40.2) -- (121,80.2) -- (81,80.2) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (101,40.2) -- (101,80.2) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (81,60.2) -- (121,60.2) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (81,40.2) -- (121,40.2) -- (121,80.2) -- (81,80.2) -- cycle ;
%Straight Lines [id:da18920070241063125] 
\draw [line width=1.5]    (121,60.2) -- (101,40.2) ;
%Straight Lines [id:da5462871111380272] 
\draw [line width=1.5]    (81,80.2) -- (101,40.2) ;
%Straight Lines [id:da5963241764049427] 
\draw [line width=1.5]    (121,60.2) -- (81,80.2) ;
%Shape: Circle [id:dp4219276121088491] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (78.9,80.2) .. controls (78.9,79.04) and (79.84,78.1) .. (81,78.1) .. controls (82.16,78.1) and (83.1,79.04) .. (83.1,80.2) .. controls (83.1,81.36) and (82.16,82.3) .. (81,82.3) .. controls (79.84,82.3) and (78.9,81.36) .. (78.9,80.2) -- cycle ;
%Shape: Circle [id:dp21278215577455395] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (98.9,80.2) .. controls (98.9,79.04) and (99.84,78.1) .. (101,78.1) .. controls (102.16,78.1) and (103.1,79.04) .. (103.1,80.2) .. controls (103.1,81.36) and (102.16,82.3) .. (101,82.3) .. controls (99.84,82.3) and (98.9,81.36) .. (98.9,80.2) -- cycle ;
%Shape: Circle [id:dp8048087935286099] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (118.9,80.2) .. controls (118.9,79.04) and (119.84,78.1) .. (121,78.1) .. controls (122.16,78.1) and (123.1,79.04) .. (123.1,80.2) .. controls (123.1,81.36) and (122.16,82.3) .. (121,82.3) .. controls (119.84,82.3) and (118.9,81.36) .. (118.9,80.2) -- cycle ;
%Shape: Circle [id:dp17092423654610078] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (78.9,60.2) .. controls (78.9,59.04) and (79.84,58.1) .. (81,58.1) .. controls (82.16,58.1) and (83.1,59.04) .. (83.1,60.2) .. controls (83.1,61.36) and (82.16,62.3) .. (81,62.3) .. controls (79.84,62.3) and (78.9,61.36) .. (78.9,60.2) -- cycle ;
%Shape: Circle [id:dp6336603977498647] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (98.9,60.2) .. controls (98.9,59.04) and (99.84,58.1) .. (101,58.1) .. controls (102.16,58.1) and (103.1,59.04) .. (103.1,60.2) .. controls (103.1,61.36) and (102.16,62.3) .. (101,62.3) .. controls (99.84,62.3) and (98.9,61.36) .. (98.9,60.2) -- cycle ;
%Shape: Circle [id:dp7358218471806388] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (118.9,60.2) .. controls (118.9,59.04) and (119.84,58.1) .. (121,58.1) .. controls (122.16,58.1) and (123.1,59.04) .. (123.1,60.2) .. controls (123.1,61.36) and (122.16,62.3) .. (121,62.3) .. controls (119.84,62.3) and (118.9,61.36) .. (118.9,60.2) -- cycle ;
%Shape: Circle [id:dp9136900028271824] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (78.9,40.2) .. controls (78.9,39.04) and (79.84,38.1) .. (81,38.1) .. controls (82.16,38.1) and (83.1,39.04) .. (83.1,40.2) .. controls (83.1,41.36) and (82.16,42.3) .. (81,42.3) .. controls (79.84,42.3) and (78.9,41.36) .. (78.9,40.2) -- cycle ;
%Shape: Circle [id:dp6403391554275268] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (98.9,40.2) .. controls (98.9,39.04) and (99.84,38.1) .. (101,38.1) .. controls (102.16,38.1) and (103.1,39.04) .. (103.1,40.2) .. controls (103.1,41.36) and (102.16,42.3) .. (101,42.3) .. controls (99.84,42.3) and (98.9,41.36) .. (98.9,40.2) -- cycle ;
%Shape: Circle [id:dp5797229117828999] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (118.9,40.2) .. controls (118.9,39.04) and (119.84,38.1) .. (121,38.1) .. controls (122.16,38.1) and (123.1,39.04) .. (123.1,40.2) .. controls (123.1,41.36) and (122.16,42.3) .. (121,42.3) .. controls (119.84,42.3) and (118.9,41.36) .. (118.9,40.2) -- cycle ;
%Shape: Grid [id:dp17507676872771727] 
\draw  [draw opacity=0] (160,40.2) -- (200,40.2) -- (200,80.2) -- (160,80.2) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (180,40.2) -- (180,80.2) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (160,60.2) -- (200,60.2) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (160,40.2) -- (200,40.2) -- (200,80.2) -- (160,80.2) -- cycle ;
%Straight Lines [id:da3524686003766009] 
\draw [line width=1.5]    (200,80.2) -- (180,40.2) ;
%Straight Lines [id:da12955800804815598] 
\draw [line width=1.5]    (160,80.2) -- (180,40.2) ;
%Straight Lines [id:da34746135952230417] 
\draw [line width=1.5]    (200,80.2) -- (160,80.2) ;
%Shape: Circle [id:dp7009694327917622] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (157.9,80.2) .. controls (157.9,79.04) and (158.84,78.1) .. (160,78.1) .. controls (161.16,78.1) and (162.1,79.04) .. (162.1,80.2) .. controls (162.1,81.36) and (161.16,82.3) .. (160,82.3) .. controls (158.84,82.3) and (157.9,81.36) .. (157.9,80.2) -- cycle ;
%Shape: Circle [id:dp02768658687912673] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (177.9,80.2) .. controls (177.9,79.04) and (178.84,78.1) .. (180,78.1) .. controls (181.16,78.1) and (182.1,79.04) .. (182.1,80.2) .. controls (182.1,81.36) and (181.16,82.3) .. (180,82.3) .. controls (178.84,82.3) and (177.9,81.36) .. (177.9,80.2) -- cycle ;
%Shape: Circle [id:dp22188276642163896] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (197.9,80.2) .. controls (197.9,79.04) and (198.84,78.1) .. (200,78.1) .. controls (201.16,78.1) and (202.1,79.04) .. (202.1,80.2) .. controls (202.1,81.36) and (201.16,82.3) .. (200,82.3) .. controls (198.84,82.3) and (197.9,81.36) .. (197.9,80.2) -- cycle ;
%Shape: Circle [id:dp39333896125569057] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (157.9,60.2) .. controls (157.9,59.04) and (158.84,58.1) .. (160,58.1) .. controls (161.16,58.1) and (162.1,59.04) .. (162.1,60.2) .. controls (162.1,61.36) and (161.16,62.3) .. (160,62.3) .. controls (158.84,62.3) and (157.9,61.36) .. (157.9,60.2) -- cycle ;
%Shape: Circle [id:dp20366709324158694] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (177.9,60.2) .. controls (177.9,59.04) and (178.84,58.1) .. (180,58.1) .. controls (181.16,58.1) and (182.1,59.04) .. (182.1,60.2) .. controls (182.1,61.36) and (181.16,62.3) .. (180,62.3) .. controls (178.84,62.3) and (177.9,61.36) .. (177.9,60.2) -- cycle ;
%Shape: Circle [id:dp0052954339361726] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (197.9,60.2) .. controls (197.9,59.04) and (198.84,58.1) .. (200,58.1) .. controls (201.16,58.1) and (202.1,59.04) .. (202.1,60.2) .. controls (202.1,61.36) and (201.16,62.3) .. (200,62.3) .. controls (198.84,62.3) and (197.9,61.36) .. (197.9,60.2) -- cycle ;
%Shape: Circle [id:dp9462322924606585] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (157.9,40.2) .. controls (157.9,39.04) and (158.84,38.1) .. (160,38.1) .. controls (161.16,38.1) and (162.1,39.04) .. (162.1,40.2) .. controls (162.1,41.36) and (161.16,42.3) .. (160,42.3) .. controls (158.84,42.3) and (157.9,41.36) .. (157.9,40.2) -- cycle ;
%Shape: Circle [id:dp4822233356931753] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (177.9,40.2) .. controls (177.9,39.04) and (178.84,38.1) .. (180,38.1) .. controls (181.16,38.1) and (182.1,39.04) .. (182.1,40.2) .. controls (182.1,41.36) and (181.16,42.3) .. (180,42.3) .. controls (178.84,42.3) and (177.9,41.36) .. (177.9,40.2) -- cycle ;
%Shape: Circle [id:dp82107071368829] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (197.9,40.2) .. controls (197.9,39.04) and (198.84,38.1) .. (200,38.1) .. controls (201.16,38.1) and (202.1,39.04) .. (202.1,40.2) .. controls (202.1,41.36) and (201.16,42.3) .. (200,42.3) .. controls (198.84,42.3) and (197.9,41.36) .. (197.9,40.2) -- cycle ;
%Shape: Grid [id:dp1307638039730472] 
\draw  [draw opacity=0] (239.5,39.7) -- (279.5,39.7) -- (279.5,79.7) -- (239.5,79.7) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (259.5,39.7) -- (259.5,79.7) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (239.5,59.7) -- (279.5,59.7) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (239.5,39.7) -- (279.5,39.7) -- (279.5,79.7) -- (239.5,79.7) -- cycle ;
%Straight Lines [id:da16917841273192624] 
\draw [line width=1.5]    (279.5,59.7) -- (259.5,39.7) ;
%Straight Lines [id:da2670815356132994] 
\draw [line width=1.5]    (239.5,59.7) -- (259.5,39.7) ;
%Straight Lines [id:da02753310283228716] 
\draw [line width=1.5]    (279.5,59.7) -- (259.5,79.7) ;
%Shape: Circle [id:dp7979688118586166] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (237.4,79.7) .. controls (237.4,78.54) and (238.34,77.6) .. (239.5,77.6) .. controls (240.66,77.6) and (241.6,78.54) .. (241.6,79.7) .. controls (241.6,80.86) and (240.66,81.8) .. (239.5,81.8) .. controls (238.34,81.8) and (237.4,80.86) .. (237.4,79.7) -- cycle ;
%Shape: Circle [id:dp9754942892802505] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (257.4,79.7) .. controls (257.4,78.54) and (258.34,77.6) .. (259.5,77.6) .. controls (260.66,77.6) and (261.6,78.54) .. (261.6,79.7) .. controls (261.6,80.86) and (260.66,81.8) .. (259.5,81.8) .. controls (258.34,81.8) and (257.4,80.86) .. (257.4,79.7) -- cycle ;
%Shape: Circle [id:dp24196744340565357] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (277.4,79.7) .. controls (277.4,78.54) and (278.34,77.6) .. (279.5,77.6) .. controls (280.66,77.6) and (281.6,78.54) .. (281.6,79.7) .. controls (281.6,80.86) and (280.66,81.8) .. (279.5,81.8) .. controls (278.34,81.8) and (277.4,80.86) .. (277.4,79.7) -- cycle ;
%Shape: Circle [id:dp6942128492517461] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (237.4,59.7) .. controls (237.4,58.54) and (238.34,57.6) .. (239.5,57.6) .. controls (240.66,57.6) and (241.6,58.54) .. (241.6,59.7) .. controls (241.6,60.86) and (240.66,61.8) .. (239.5,61.8) .. controls (238.34,61.8) and (237.4,60.86) .. (237.4,59.7) -- cycle ;
%Shape: Circle [id:dp020458523873414514] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (257.4,59.7) .. controls (257.4,58.54) and (258.34,57.6) .. (259.5,57.6) .. controls (260.66,57.6) and (261.6,58.54) .. (261.6,59.7) .. controls (261.6,60.86) and (260.66,61.8) .. (259.5,61.8) .. controls (258.34,61.8) and (257.4,60.86) .. (257.4,59.7) -- cycle ;
%Shape: Circle [id:dp17745358958001511] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (277.4,59.7) .. controls (277.4,58.54) and (278.34,57.6) .. (279.5,57.6) .. controls (280.66,57.6) and (281.6,58.54) .. (281.6,59.7) .. controls (281.6,60.86) and (280.66,61.8) .. (279.5,61.8) .. controls (278.34,61.8) and (277.4,60.86) .. (277.4,59.7) -- cycle ;
%Shape: Circle [id:dp3390757435061216] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (237.4,39.7) .. controls (237.4,38.54) and (238.34,37.6) .. (239.5,37.6) .. controls (240.66,37.6) and (241.6,38.54) .. (241.6,39.7) .. controls (241.6,40.86) and (240.66,41.8) .. (239.5,41.8) .. controls (238.34,41.8) and (237.4,40.86) .. (237.4,39.7) -- cycle ;
%Shape: Circle [id:dp5048172448800725] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (257.4,39.7) .. controls (257.4,38.54) and (258.34,37.6) .. (259.5,37.6) .. controls (260.66,37.6) and (261.6,38.54) .. (261.6,39.7) .. controls (261.6,40.86) and (260.66,41.8) .. (259.5,41.8) .. controls (258.34,41.8) and (257.4,40.86) .. (257.4,39.7) -- cycle ;
%Shape: Circle [id:dp43350502524911594] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (277.4,39.7) .. controls (277.4,38.54) and (278.34,37.6) .. (279.5,37.6) .. controls (280.66,37.6) and (281.6,38.54) .. (281.6,39.7) .. controls (281.6,40.86) and (280.66,41.8) .. (279.5,41.8) .. controls (278.34,41.8) and (277.4,40.86) .. (277.4,39.7) -- cycle ;
%Straight Lines [id:da4382976520650499] 
\draw [line width=1.5]    (259.5,79.7) -- (239.5,59.7) ;
%Shape: Circle [id:dp2841583324016317] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (85.4,47.7) .. controls (85.4,46.54) and (86.34,45.6) .. (87.5,45.6) .. controls (88.66,45.6) and (89.6,46.54) .. (89.6,47.7) .. controls (89.6,48.86) and (88.66,49.8) .. (87.5,49.8) .. controls (86.34,49.8) and (85.4,48.86) .. (85.4,47.7) -- cycle ;
%Shape: Circle [id:dp6880255687313708] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (92.4,53.7) .. controls (92.4,52.54) and (93.34,51.6) .. (94.5,51.6) .. controls (95.66,51.6) and (96.6,52.54) .. (96.6,53.7) .. controls (96.6,54.86) and (95.66,55.8) .. (94.5,55.8) .. controls (93.34,55.8) and (92.4,54.86) .. (92.4,53.7) -- cycle ;
%Shape: Circle [id:dp5237692348302281] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (105.4,47.2) .. controls (105.4,46.04) and (106.34,45.1) .. (107.5,45.1) .. controls (108.66,45.1) and (109.6,46.04) .. (109.6,47.2) .. controls (109.6,48.36) and (108.66,49.3) .. (107.5,49.3) .. controls (106.34,49.3) and (105.4,48.36) .. (105.4,47.2) -- cycle ;
%Shape: Circle [id:dp16100722772310805] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (112.4,53.2) .. controls (112.4,52.04) and (113.34,51.1) .. (114.5,51.1) .. controls (115.66,51.1) and (116.6,52.04) .. (116.6,53.2) .. controls (116.6,54.36) and (115.66,55.3) .. (114.5,55.3) .. controls (113.34,55.3) and (112.4,54.36) .. (112.4,53.2) -- cycle ;
%Shape: Circle [id:dp46551009120635767] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (105.4,67.2) .. controls (105.4,66.04) and (106.34,65.1) .. (107.5,65.1) .. controls (108.66,65.1) and (109.6,66.04) .. (109.6,67.2) .. controls (109.6,68.36) and (108.66,69.3) .. (107.5,69.3) .. controls (106.34,69.3) and (105.4,68.36) .. (105.4,67.2) -- cycle ;
%Shape: Circle [id:dp5824446201721556] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (112.4,73.2) .. controls (112.4,72.04) and (113.34,71.1) .. (114.5,71.1) .. controls (115.66,71.1) and (116.6,72.04) .. (116.6,73.2) .. controls (116.6,74.36) and (115.66,75.3) .. (114.5,75.3) .. controls (113.34,75.3) and (112.4,74.36) .. (112.4,73.2) -- cycle ;
%Shape: Circle [id:dp6308683740642695] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (84.9,67.7) .. controls (84.9,66.54) and (85.84,65.6) .. (87,65.6) .. controls (88.16,65.6) and (89.1,66.54) .. (89.1,67.7) .. controls (89.1,68.86) and (88.16,69.8) .. (87,69.8) .. controls (85.84,69.8) and (84.9,68.86) .. (84.9,67.7) -- cycle ;
%Shape: Circle [id:dp2577554202225387] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (91.9,73.7) .. controls (91.9,72.54) and (92.84,71.6) .. (94,71.6) .. controls (95.16,71.6) and (96.1,72.54) .. (96.1,73.7) .. controls (96.1,74.86) and (95.16,75.8) .. (94,75.8) .. controls (92.84,75.8) and (91.9,74.86) .. (91.9,73.7) -- cycle ;
%Shape: Circle [id:dp6943750313533943] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (167.9,60.2) .. controls (167.9,59.04) and (168.84,58.1) .. (170,58.1) .. controls (171.16,58.1) and (172.1,59.04) .. (172.1,60.2) .. controls (172.1,61.36) and (171.16,62.3) .. (170,62.3) .. controls (168.84,62.3) and (167.9,61.36) .. (167.9,60.2) -- cycle ;
%Shape: Circle [id:dp6530140699170282] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (187.9,80.2) .. controls (187.9,79.04) and (188.84,78.1) .. (190,78.1) .. controls (191.16,78.1) and (192.1,79.04) .. (192.1,80.2) .. controls (192.1,81.36) and (191.16,82.3) .. (190,82.3) .. controls (188.84,82.3) and (187.9,81.36) .. (187.9,80.2) -- cycle ;
%Shape: Circle [id:dp1759587949946675] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (187.9,60.2) .. controls (187.9,59.04) and (188.84,58.1) .. (190,58.1) .. controls (191.16,58.1) and (192.1,59.04) .. (192.1,60.2) .. controls (192.1,61.36) and (191.16,62.3) .. (190,62.3) .. controls (188.84,62.3) and (187.9,61.36) .. (187.9,60.2) -- cycle ;
%Shape: Circle [id:dp7996006122272241] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (168.4,80.2) .. controls (168.4,79.04) and (169.34,78.1) .. (170.5,78.1) .. controls (171.66,78.1) and (172.6,79.04) .. (172.6,80.2) .. controls (172.6,81.36) and (171.66,82.3) .. (170.5,82.3) .. controls (169.34,82.3) and (168.4,81.36) .. (168.4,80.2) -- cycle ;
%Shape: Circle [id:dp6916719228355583] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (187.4,40.2) .. controls (187.4,39.04) and (188.34,38.1) .. (189.5,38.1) .. controls (190.66,38.1) and (191.6,39.04) .. (191.6,40.2) .. controls (191.6,41.36) and (190.66,42.3) .. (189.5,42.3) .. controls (188.34,42.3) and (187.4,41.36) .. (187.4,40.2) -- cycle ;
%Shape: Circle [id:dp14024362676541546] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (167.4,40.2) .. controls (167.4,39.04) and (168.34,38.1) .. (169.5,38.1) .. controls (170.66,38.1) and (171.6,39.04) .. (171.6,40.2) .. controls (171.6,41.36) and (170.66,42.3) .. (169.5,42.3) .. controls (168.34,42.3) and (167.4,41.36) .. (167.4,40.2) -- cycle ;
%Shape: Circle [id:dp13489246888722506] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (247.4,49.7) .. controls (247.4,48.54) and (248.34,47.6) .. (249.5,47.6) .. controls (250.66,47.6) and (251.6,48.54) .. (251.6,49.7) .. controls (251.6,50.86) and (250.66,51.8) .. (249.5,51.8) .. controls (248.34,51.8) and (247.4,50.86) .. (247.4,49.7) -- cycle ;
%Shape: Circle [id:dp14171475661526367] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (267.4,69.7) .. controls (267.4,68.54) and (268.34,67.6) .. (269.5,67.6) .. controls (270.66,67.6) and (271.6,68.54) .. (271.6,69.7) .. controls (271.6,70.86) and (270.66,71.8) .. (269.5,71.8) .. controls (268.34,71.8) and (267.4,70.86) .. (267.4,69.7) -- cycle ;
%Shape: Circle [id:dp735720385855146] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (267.4,49.7) .. controls (267.4,48.54) and (268.34,47.6) .. (269.5,47.6) .. controls (270.66,47.6) and (271.6,48.54) .. (271.6,49.7) .. controls (271.6,50.86) and (270.66,51.8) .. (269.5,51.8) .. controls (268.34,51.8) and (267.4,50.86) .. (267.4,49.7) -- cycle ;
%Shape: Circle [id:dp3180532995319263] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 0; blue, 0 }  ,fill opacity=1 ] (247.4,69.7) .. controls (247.4,68.54) and (248.34,67.6) .. (249.5,67.6) .. controls (250.66,67.6) and (251.6,68.54) .. (251.6,69.7) .. controls (251.6,70.86) and (250.66,71.8) .. (249.5,71.8) .. controls (248.34,71.8) and (247.4,70.86) .. (247.4,69.7) -- cycle ;
\end{tikzpicture}
    \caption{The polygons No.16, 13 and 15 (in black) on the lattice. After refine the lattices by adding the red points in the plots, we get their dual polygons (No.1, 2 and 4) in the new lattices.}\label{latticerefinement}
\end{figure}

In particular, for the three polygons here, they become their dual polygons after the refinements of lattices as follows:
\begin{equation}
    \begin{split}
        \text{No.}16\mapsto\text{No.}1&:~\mathbb{Z}^3\mapsto\mathbb{Z}^3+{\color{red}\frac{1}{3}(0,1,2)}\mathbb{Z}^3,\\
        \text{No.}13\mapsto\text{No.}2&:~\mathbb{Z}^3\mapsto\mathbb{Z}^3+{\color{red}(0,1,0)}\mathbb{Z}^3,\\
        \text{No.}15\mapsto\text{No.}5&:~\mathbb{Z}^3\mapsto\mathbb{Z}^3+{\color{red}\frac{1}{2}(0,1,1)}\mathbb{Z}^3,
    \end{split}
\end{equation}
where we have used $\mathbb{Z}^3$ as these polygons are the coplanar endpoints of the 3d cones for the corresponding CY 3-folds. The red parts are called the quotient gradings\footnote{Notice that however it is possible to have more than one choices to relate two polygons by quotient gradings. Hence, this is not canonically defined.}, and we may write $\text{No.}1=\text{No.}16/\frac{1}{3}(0,1,2)$ etc. However, on the other hand, each dual pair in the remaining 9 polygons do not enjoy this property.

This can be more quickly verified by their Pl\"ucker coordinates obtained as follows. We first write the vertices of a lattice polygon as a matrix. Then the kernel of this matrix, which itself is a matrix of size $r\times n$ ($r\leq n$), is known as the grading since it reveals the linear relations among the vertices. Now the $r\times r$ minors of the grading matrix forms some homogeneous coordinates known as the Pl\"ucker coordinates\footnote{Hence, there are $2n!$ equivalent ways to write the Pl\"ucker coordinates for a lattice polytope with $n$ vertices due to different orderings in the matrix, where $n!$ comes from the symmetric group $\mathfrak{S}_n$ for permuting vertices and the factor 2 indicates an overall sign. Although we have this freedom in writing Pl\"ucker coordinates, the precise values of entries would not change up to ordering and the overall sign.}. For the polygons (including their duals) in Figure \ref{latticerefinement}, each pair has the same Pl\"ucker coordinates respectively:
\begin{equation}
    \text{No.}1\&16:(1:1:1),~~\text{No.}2\&13:(2:1:1),~~\text{No.}4\&15:(1:0:1:-1:0:1).
\end{equation}
Incidentally, we may also write the Pl\"ucker coordinates for polygon No.7 here: $(2:1:3)$. As a matter of fact, it is not hard to check that the Pl\"ucker coordinates are GL$(2,\mathbb{Z})$ invariant. Hence, different polygons can have same Pl\"ucker coordinates and they are related by the quotient gradings discussed above.

For reference, we list the Pl\"ucker coordinates for the remaining 9 polygons as well:
\begin{equation}
    \begin{split}
            &\text{No.}3:(2:1:3:-1:1:2),~~~~~~~~~~~~~~~~~~~~~~~~\text{No.}14:(1:0:1:-1:-1:1),\\
            &\text{No.}5:(2:1:3:-1:-1:1),~~~~~~~~~~~~~~~~~~~~~~\text{No.}11:(2:-1:1:-1:-1:1),\\
            &\text{No.}6:(2:-1:1:-1:-1:1:2:0:-1:1),~\text{No.}12:(1:-1:1:0:-1:1:1:0:-1:1),\\
            &\text{No.}8:(2:-1:1:-2:0:1),\\
            &\text{No.}9:(1:-1:1:0:-1:1:1:0:-1:1),\\
            &\text{No.}10:(1:-1:1:0:-1:1:1:0:-1:1:-1:1:0:-1:1),
    \end{split}
\end{equation}
where the dual polygons are arranged in the same rows. As we can see, they all have different Pl\"ucker coordinates and hence not related by quotient gradings. It is now straightforward to tell whether any polygons are related by GL$(2,\mathbb{Z})$ transformations or not. Thus, this explains why only the 4 special classes have the same respective Mahler measures (and periods) while the others do not.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Surface Tension and Quiver Entropy}
\rem{The main question in this section is about the space of the all possible values (moduli space) of the Mahler measure. We claim that the space of possible values of the Mahler measure is the surface tension of the dimer model given by the Legendre dual of the Ronkin function. For a review on the statistical physics of the toric dimer model see \cite{bocklandt2016dimer}. This space is a continuous convex surface with a (conical) singularity at the internal point of the toric diagram, when the gas phase opens, otherwise it is smooth and differentible everywhere. The sharpness of the peak of the surface tension depends on the $k$ and the size of the hole.
In order to prove the relation between the Mahler measure and surface tension, we need to find the map between the $R$-charges (isoradial angles $\theta_I$'s) and the slopes $(s,t)$. For this, we need to show that the possible $R$-charges (isoradial angles $\theta_I$'s), similar to $(s,t)$, take value from the toric diagram. In fact, only if we can find the map explicitly, then we can claim that the surface tension of the dimer model is the quiver entropy.}

\rem{The moduli space of (NP of) a geometrically fixed dimer model but with different weights is the moduli space of the Harnack curves. In fact, by varying the edge weights all Harnack curves can be obtained as the characteristic polynomials of the dimer model. Especially, the isoradial dimer models are characterized by the genus zero Harnack curves.}
\rem{The space of all possible characteristic polynomials and thus all possible Mahler measures is the moduli space of the Harnack curves}
\rem{The set of gauge invariant edge weights of the dimer model are in bijection with the set of K\"ahler parameters $\{t_i\}$ and the coordinates $(x,y)$ or their Legendre dual $(s,t)$, i.e. the slopes of the dimer model.}

\paragraph{RG space}

The full RG space of the toric quiver gauge theory is a space that the quiver flows from the space of isoradial theories to a unique tropical theory. The RG space can be characterized via the three parameters, i.e. K\"ahler parameter $k$ and the slope parameters $(s,t)$. We can divide the RG flow to two categories. One is the RG flow inside the two-dimensional space $\sigma(s,t)$ at any fixed $k$ with the fixed point corresponding to the extremized Mahler measure, and the second one is the RG flow of the $\sigma(s,t)$ (possibly singular) surface as we change $k$ from $k_{\text{iso}}$ to $k_{\text{trop}}=\infty$. The evolution of the $\sigma_k(s,t)$ surface from a smooth differentiable manifold at $k_{\text{iso}}$ to a manifold with conical singularity for $k_{\text{iso}}<k<k_{\text{trop}}$ and finally to a singular point $\sigma=\log k$, at $k_{\text{trop}}$ can be completely determined. The dynamics of the surface tension for a fixed $k$ is determined by the Monge-Amp\`ere equation \cite{Kenyon:2003uj,passare2000amoebas}.

\subsubsection*{Minimal set of coefficients of the Mahler measure and dimer model}
There is a space of generalized Mahler measure with minimal (physical) set of coefficients in the space of all possible generalized Mahler measure with arbitrary coefficients. This particular minimal set, reduces the generalized Mahler measure to the Ronkin function of the dimer model.

For any fixed value of the K\"{a}hler parameter, especially at $k_{\text{iso}}$, the remaining degrees of freedom (d.o.f) are the $(x,y)$ coordinates of the Ronkin function, which are the dual coordinates to the $(s,t)$ coordinates of the surface tension. Thus, assuming the map between $R$-charges and $(s,t)$, we can confer that at fixed K\"{a}hler parameter, we naturally have the d.o.f as trial $R$-charges. 


\rem{Another conjecture that we may be able to prove is about the moduli space of all possible $R$-charges (rhombus angles $\theta$'s). In the language of dimer model, the moduli space of trial $R$-charges is the toric diagram and the space of all possible Mahler measure is the two-dimensional smooth convex manifold defined by the surface tension $\sigma(s,t)$, the Legendre dual of the Ronkin function $R(x,y)$.}

The quiver asymptotic analysis includes computation of the height function (Ronkin function), the entropy and the growth rate (Mahler measure). Entropy function determines the degeneracy of the D-brane bound states of the CY, crystal,...
In this part, we compte the Ronkin function and entropy of the quiver at isoradial/non-isoradial cases.

The entropy function is defined as the Legendre transform of the Ronkin function
\bea
\sigma(s,t) = -R(x,y) +s\, x+ t\, y,\qquad \text{where}\qquad (s,t) = \nabla R (x,y).
\eea
$(s,t)$ are the slopes functions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Appendices for reflexives
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Examples: Mahler Measures for Reflexive Polygons}\label{mahlerlist}
Following the ordering in \cite[Figure 1 and 2]{Hanany:2012hi}, $P(z,w)=k-p(z,w)$, $m(P)$ and $u_0(k)$ for the 16 reflexive polygons are
\paragraph{1. $\mathbb{C}^3/(\mathbb{Z}_3\times\mathbb{Z}_3)$ $(1,0,2)(0,1,2)$:}
\begin{equation}
    P=-z^2w^{-1}-z^{-1}w^2-z^{-1}w^{-1}-3z^{-1}w-3z^{-1}-3w^{-1}-3z-3w+k,
\end{equation}
with $k\geq k_\text{iso}=21$;
\begin{equation}
    \begin{split}
        m(P)=&\log k-\frac{27}{k^2}-\frac{164}{k^3}-\frac{4941}{2k^4}-\frac{31752}{k^5}-\frac{479940}{k^6}-\frac{7426080}{k^7}-\frac{482173965}{4k^8}\\
        &-\frac{6030521840}{3k^9}-\frac{171779570802}{k^{10}}-\dots,
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        u_0(k)=&1+\frac{54}{k^2}+\frac{492}{k^3}+\frac{9882}{k^4}+\frac{158760}{k^5}+\frac{2879640}{k^6}+\frac{51982560}{k^7}+\frac{964347930}{k^8}\\
        &+\frac{18091565520}{k^9}+\frac{343559141604}{k^{10}}+\dots
    \end{split}
\end{equation}
for $k\geq p(1,1)=21$, and when $k=k_\text{iso}=21$,
\begin{equation}
    m(P)=-\frac{3i\left(\pi^2+18\text{Li}_2\left(\frac{-1+i\sqrt{3}}{2}\right)\right)}{4\pi}\approx2.90759;
\end{equation}
\paragraph{2. $\mathbb{C}^3/(\mathbb{Z}_4\times\mathbb{Z}_2)$ $(1,0,3)(0,1,1)$:}
\begin{equation}
    P=-zw-zw^{-1}-z^{-3}w^{-1}-2z-2z^{-1}-4w^{-1}-6z^{-1}w^{-1}-4z^{-2}w^{-1}+k
\end{equation}
with $k\geq k_\text{iso}=12$;
\begin{equation}
    \begin{split}
        m(P)=&\log k-\frac{10}{k^2}-\frac{32}{k^3}-\frac{297}{k^4}-\frac{2112}{k^5}-\frac{55720}{3k^6}-\frac{163200}{k^7}-\frac{3038665}{2k^8}\\
        &-\frac{43406720}{3k^9}-\frac{141433992}{k^{10}}-\dots,
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        u_0(k)=&1+\frac{20}{k^2}+\frac{96}{k^3}+\frac{1188}{k^4}+\frac{10560}{k^5}+\frac{111440}{k^6}+\frac{1142400}{k^7}+\frac{12154660}{k^8}\\
        &+\frac{130220160}{k^9}+\frac{1414339920}{k^{10}}+\dots
    \end{split}
\end{equation}
for $k\geq p(1,1)=21$, and when $k=k_\text{iso}=12$,
\begin{equation}
    m(P)=-\frac{2i\left(\pi^2+18\text{Li}_2\left(\frac{-1+i\sqrt{3}}{2}\right)\right)}{3\pi}\approx2.58453;
\end{equation}
\paragraph{3. $L^{1,3,1}/\mathbb{Z}_2$ $(0,1,1,1)$:}
\begin{equation}
    P=-\frac{AB}{C}(zw+w)-\frac{C}{AB}(zw^{-1}+z^{-2}w^{-1}+3w^{-1}+3z^{-1}w^{-1})-(2z+2z^{-1})+k,
\end{equation}
where
\begin{equation}
    A=\sin\left(\frac{5-\sqrt{7}}{12}\pi\right),B=\sin^2\left(\frac{5-\sqrt{7}}{6}\pi\right),C=\sin^3\left(\frac{1+\sqrt{7}}{12}\pi\right),
\end{equation}
with $k\geq k_\text{iso}=12$;
\begin{equation}
    \begin{split}
        m(P)=&\log k-\frac{10}{k^2}-\frac{32}{k^3}-\frac{297}{k^4}-\frac{2112}{k^5}-\frac{55720}{3k^6}-\frac{163200}{k^7}-\frac{3038665}{2k^8}\\
        &-\frac{43406720}{3k^9}-\frac{141433992}{k^{10}}-\dots,
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        u_0(k)=&1+\frac{20}{k^2}+\frac{96}{k^3}+\frac{1188}{k^4}+\frac{10560}{k^5}+\frac{111440}{k^6}+\frac{1142400}{k^7}+\frac{12154660}{k^8}\\
        &+\frac{130220160}{k^9}+\frac{1414339920}{k^{10}}+\dots
    \end{split}
\end{equation}
for $k\geq p(1,1)=\frac{2AB}{C}+\frac{8C}{AB}+4\approx14.3492$, and when $k=k_\text{iso}=12$,
\begin{equation}
    \begin{split}
        m(P)=&\frac{2-\sqrt{7}}{18}\left(11i\pi+6\log\left(\cos\left(\frac{1+\sqrt{7}}{12}\pi\right)\right)+18\log\left(\csc\left(\frac{1+\sqrt{7}}{12}\pi\right)\right)\right.\\
        &\left.+12\log\left(\sin\left(\frac{1+\sqrt{7}}{6}\pi\right)\right)\right)-\frac{2i}{\pi}\left(\text{Li}_2\left(\text{e}^{i\frac{5-\sqrt{7}}{6}\pi}\right)+\text{Li}_2\left(\text{e}^{i\frac{5-\sqrt{7}}{3}\pi}\right)+3\text{Li}_2\left(\text{e}^{i\frac{1+\sqrt{7}}{6}\pi}\right)\right)\\
        \approx&2.41581;
    \end{split}
\end{equation}
\paragraph{4. $\mathcal{C}/(\mathbb{Z}_2\times\mathbb{Z}_2)$ $(1,0,0,1)(0,1,1,0)$:}
\begin{equation}
    P=-zw^{-1}-z^{-1}w^{-1}-z^{-1}w-zw-2z-2z^{-1}-2w-2w^{-1}+k
\end{equation}
with $k\geq k_\text{iso}=12$;
\begin{equation}
    \begin{split}
        m(P)=&\log k-\frac{27}{k^2}-\frac{164}{k^3}-\frac{4941}{2k^4}-\frac{31752}{k^5}-\frac{479940}{k^6}-\frac{7426080}{k^7}-\frac{482173965}{4k^8}\\
        &-\frac{6030521840}{3k^9}-\frac{171779570802}{k^{10}}-\dots,
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        u_0(k)=&1+\frac{54}{k^2}+\frac{492}{k^3}+\frac{9882}{k^4}+\frac{158760}{k^5}+\frac{2879640}{k^6}+\frac{51982560}{k^7}+\frac{964347930}{k^8}\\
        &+\frac{18091565520}{k^9}+\frac{343559141604}{k^{10}}+\dots
    \end{split}
\end{equation}
for $k\geq p(1,1)=12$, and when $k=k_\text{iso}=12$,
\begin{equation}
    m(P)=\frac{8\mathcal{K}}{\pi}\approx2.33249;
\end{equation}
\paragraph{5. PdP$_{4b}$:}
\begin{equation}
    \begin{split}
        P=&-\frac{A_1A_2A_3^2}{A_5A_6}z-\frac{A_3^2A_4^3}{A_1A_5A_6}zw^{-1}-\frac{A_5^5}{A_1A_3A_6}z^{-2}w^{-1}-\frac{A_1A_6^3}{A_3A_5}w-\frac{2A_5^2A_6}{A_3}z^{-1}\\
        &-\frac{3A_3A_4^2A_5}{A_1A_6}w^{-1}-\frac{3A_4A_5^3}{A_1A_6}z^{-1}w^{-1}+k
    \end{split}
\end{equation}
with $k\geq k_\text{iso}=\frac{2A_4^2A_6^2}{A_1A_3}+\frac{A_2A_4A_5A_6}{A_1A_3}+2A_1A_3+2A_2A_5+2A_4A_6\approx4.59623$, where $A_i=\sin(\pi a_i/2)$ and
\begin{equation}
    \begin{split}
        &a_1\approx0.821\text{ is a root of }27x^4-108x^3+36x^2+116x-72=0;\\
        &a_2\approx0.243\text{ is a root of }27x^4+54x^3-432x^2+496x-96=0;\\
        &a_3\approx0.783\text{ is a root of }81x^4-324x^3+288x^2+16x-64=0;\\
        &a_4\approx0.539\text{ is a root of }81x^4-486x^3+288x^2+448x-256=0;\\
        &a_5\approx0.640\text{ is a root of }81x^4+162x^3-36x^2-52x-8=0;\\
        &a_6\approx0.577\text{ is a root of }27x^4-162x^3+180x^2+28x-48=0;
    \end{split}\label{Aiai}
\end{equation}
\begin{equation}
    {\tiny \begin{split}
        m(P)=&\log k-\frac{2A_1A_2A_3A_5+3A_4^2A_6^2}{k^2}-\frac{2A_4A_6 \left(2 A_4^2 A_6^2+3 A_1 A_2 A_3 A_5\right)}{k^3}-\frac{9\left(5 A_4^4 A_6^4+8 A_1 A_2 A_3 A_4^2 A_5A_6^2+2 A_1^2 A_2^2 A_3^2 A_5^2\right)}{2 k^4}\\
        &-\frac{24A_4A_6 \left(3 A_4^4 A_6^4+7 A_1 A_2 A_3 A_4^2 A_5 A_6^2+3 A_1^2 A_2^2 A_3^2 A_5^2\right)}{k^5}-\frac{5\left(204 A_4^6 A_6^6+540 A_1 A_2 A_3 A_4^4 A_5A_6^4+351 A_1^2 A_2^2 A_3^2 A_4^2 A_5^2 A_6^2+40 A_1^3 A_2^3 A_3^3 A_5^3\right)}{3 k^6}\\
   &-\frac{60A_4A_6\left(24 A_4^6 A_6^6+78 A_1 A_2 A_3 A_4^4 A_5 A_6^4+68 A_1^2 A_2^2 A_3^2 A_4^2 A_5^2 A_6^2+15 A_1^3 A_2^3 A_3^3
   A_5^3\right)}{k^7}\\
   &-\frac{35\left(783 A_4^8 A_6^8+2880 A_1 A_2 A_3 A_4^6 A_5 A_6^6+3168 A_1^2 A_2^2 A_3^2 A_4^4 A_5^2 A_6^4+1104 A_1^3 A_2^3 A_3^3 A_4^2 A_5^3 A_6^2+70 A_1^4 A_2^4 A_3^4 A_5^4\right)}{4 k^8}\\
        &-\frac{560A_4A_6\left(173 A_4^8 A_6^8+729 A_1 A_2 A_3 A_4^6 A_5 A_6^6+972 A_1^2 A_2^2 A_3^2 A_4^4 A_5^2 A_6^4+468 A_1^3 A_2^3 A_3^3 A_4^2 A_5^3 A_6^2+63 A_1^4 A_2^4 A_3^4 A_5^4\right)}{3 k^9}\\
   &-\frac{378\left(2101A_4^{10} A_6^{10}+9850 A_1 A_2 A_3 A_4^8 A_5 A_6^8+15450 A_1^2 A_2^2 A_3^2 A_4^6 A_5^2 A_6^6+9600 A_1^3 A_2^3 A_3^3 A_4^4 A_5^3 A_6^4+2100 A_1^4 A_2^4 A_3^4 A_4^2 A_5^4 A_6^2+84 A_1^5 A_2^5 A_3^5 A_5^5\right)}{5 k^{10}}\\
   &-\dots,
    \end{split}}
\end{equation}
\begin{equation}
    {\tiny \begin{split}
        u_0(k)=&1+\frac{2\left(3 A_4^2 A_6^2+2 A_1 A_2 A_3 A_5\right)}{k^2}+\frac{6A_4A_6\left(2 A_4^2 A_6^2+3 A_1 A_2 A_3 A_5\right)}{k^3}+\frac{18\left(5 A_4^4 A_6^4+8 A_1 A_2 A_3 A_4^2 A_5
   A_6^2+2 A_1^2 A_2^2 A_3^2 A_5^2\right)}{k^4}\\
   &+\frac{120A_4A_6\left(3 A_4^4 A_6^4+7 A_1 A_2 A_3 A_4^2 A_5 A_6^2+3 A_1^2 A_2^2 A_3^2 A_5^2\right)}{k^5}+\frac{10\left(204 A_4^6 A_6^6+540 A_1 A_2 A_3 A_4^4 A_5
   A_6^4+351 A_1^2 A_2^2 A_3^2 A_4^2 A_5^2A_6^2+40A_1^3A_2^3A_3^3A_5^3\right)}{k^6}\\
   &+\frac{420A_4A_6\left(24 A_4^6 A_6^6+78 A_1 A_2 A_3 A_4^4 A_5 A_6^4+68 A_1^2 A_2^2 A_3^2 A_4^2 A_5^2 A_6^2+15 A_1^3 A_2^3 A_3^3
   A_5^3\right)}{k^7}\\
   &+\frac{70\left(783 A_4^8 A_6^8+2880 A_1 A_2 A_3 A_4^6 A_5 A_6^6+3168 A_1^2 A_2^2 A_3^2 A_4^4 A_5^2 A_6^4+1104 A_1^3 A_2^3 A_3^3 A_4^2 A_5^3 A_6^2+70 A_1^4 A_2^4 A_3^4 A_5^4\right)}{k^8}\\
    &+\frac{1680A_4A_6\left(173 A_4^8 A_6^8+729 A_1 A_2 A_3 A_4^6 A_5 A_6^6+972 A_1^2 A_2^2 A_3^2 A_4^4 A_5^2 A_6^4+468 A_1^3 A_2^3 A_3^3 A_4^2 A_5^3 A_6^2+63 A_1^4 A_2^4 A_3^4 A_5^4\right)}{k^9}\\
   &+\frac{756\left(2101A_4^{10} A_6^{10}+9850 A_1 A_2 A_3 A_4^8 A_5 A_6^8+15450 A_1^2 A_2^2 A_3^2 A_4^6 A_5^2 A_6^6+9600 A_1^3 A_2^3 A_3^3 A_4^4 A_5^3 A_6^4+2100 A_1^4 A_2^4 A_3^4 A_4^2 A_5^4 A_6^2+84 A_1^5 A_2^5 A_3^5 A_5^5\right)}{k^{10}}\\
   &+\dots
    \end{split}}
\end{equation}
for $k\geq p(1,1)\approx7.00504$, and when $k=k_\text{iso}$,
\begin{equation}
    \begin{split}
        m(P)=&-\frac{i}{2\pi}\left(2\text{Li}_2(\text{e}^{a_1})+\text{Li}_2(\text{e}^{a_2})+3\text{Li}_2(\text{e}^{a_3})+3\text{Li}_2(\text{e}^{a_4})+6\text{Li}_2(\text{e}^{a_5})+4\text{Li}_2(\text{e}^{a_6})\right)\\
        &-\frac{i\pi}{72}\mathfrak{a}_0+\frac{1}{6}(-36\log(2)+6a_1\log(1-\text{e}^{a_1})+3a_2\log(1-\text{e}^{a_2})+9a_3\log(1-\text{e}^{a_3})\\
        &+9a_4\log(1-\text{e}^{a_4})+18a_5\log(1-\text{e}^{a_5})+12a_6\log(1-\text{e}^{a_6}))-\log(A_1A_3A_5A_6)\\
        \approx&1.57265,
    \end{split}
\end{equation}
where
\begin{equation}
    \mathfrak{a}_0\approx-42.833\text{ is a root of }x^4-2208x^3+689640x^2-39837376x-3148479024=0;
\end{equation}
\paragraph{6. PdP$_{4a}$:}
\begin{equation}
    P=-B_1^2B_2^2(z+z^{-1})-B_2^2B_3B_4(zw^{-1}+w^{-1})-B_5^4z^{-1}w^2-2B_1B_2B_5^2(z^{-1}w+w)+k
\end{equation}
with $k\geq k_\text{iso}=2B_1^2B_2^2+4B_1B_2B_3B_5+2B_2^2B_4B_5+B_3^2B_5^2\approx2.53893$, where $B_i=\sin(\pi b_i/2)$ and
\begin{equation}
    \begin{split}
        &b_1\approx0.427\text{ is a root of }3x^3-340x^2-24x+72=0;\\
        &b_2\approx0.725\text{ is a root of }3x^3-134x^2+228x-96=0;\\
        &b_3\approx0.298\text{ is a root of }3x^3+206x^2-384x+96=0;\\
        &b_4\approx0.596\text{ is a root of }3x^3+412x^2-1536x+768=0;\\
        &b_5\approx0.550\text{ is a root of }3x^3+250x^2-124x-8=0;
    \end{split}
\end{equation}
\begin{equation}
    {\tiny \begin{split}
        m(P)=&\log k-\frac{B_1 B_2^3 \left(B_2 B_1^3+4 B_3 B_4 B_5^2\right)}{k^2}-\frac{2 B_2^4 B_3 B_4 B_5^2 \left(4 B_2 B_1^3+B_3 B_4 B_5^2\right)}{k^3}-\frac{3 B_1^2 B_2^6 \left(B_2^2 B_1^6+16 B_2 B_3 B_4 B_5^2 B_1^3+28 B_3^2 B_4^2 B_5^4\right)}{2 k^4}\\
        &-\frac{24 B_1
   B_2^7 B_3 B_4 B_5^2 \left(2 B_2^2 B_1^6+9 B_2 B_3 B_4 B_5^2 B_1^3+2 B_3^2 B_4^2 B_5^4\right)}{k^5}\\
   &-\frac{5 B_2^8 \left(2 B_2^4 B_1^{12}+72 B_2^3 B_3 B_4 B_5^2 B_1^9+540 B_2^2 B_3^2 B_4^2 B_5^4 B_1^6+512 B_2 B_3^3 B_4^3 B_5^6 B_1^3+9 B_3^4 B_4^4
   B_5^8\right)}{3 k^6}\\
   &-\frac{60 B_1^2 B_2^{10} B_3 B_4 B_5^2 \left(4 B_2^3 B_1^9+51 B_2^2 B_3 B_4 B_5^2 B_1^6+108 B_2 B_3^2 B_4^2 B_5^4 B_1^3+22 B_3^3 B_4^3 B_5^6\right)}{k^7}\\
   &-\frac{35 B_1 B_2^{11} \left(B_2^5 B_1^{15}+64 B_2^4 B_3 B_4 B_5^2 B_1^{12}+1104
   B_2^3 B_3^2 B_4^2 B_5^4 B_1^9+4096 B_2^2 B_3^3 B_4^3 B_5^6 B_1^6+2644 B_2 B_3^4 B_4^4 B_5^8 B_1^3+96 B_3^5 B_4^5 B_5^{10}\right)}{4 k^8}\\
        &-\frac{560 B_2^{12} B_3 B_4 B_5^2 \left(6 B_2^5 B_1^{15}+150 B_2^4 B_3 B_4 B_5^2 B_1^{12}+868 B_2^3 B_3^2 B_4^2 B_5^4
   B_1^9+1158 B_2^2 B_3^3 B_4^3 B_5^6 B_1^6+222 B_2 B_3^4 B_4^4 B_5^8 B_1^3+B_3^5 B_4^5 B_5^{10}\right)}{3 k^9}\\
   &-\frac{126 B_1^2 B_2^{14}}{5 k^{10}} \left(B_2^6 B_1^{18}+100 B_2^5 B_3 B_4 B_5^2 B_1^{15}+3100 B_2^4 B_3^2 B_4^2 B_5^4 B_1^{12}+25600 B_2^3 B_3^3 B_4^3
   B_5^6 B_1^9+58150 B_2^2 B_3^4 B_4^4 B_5^8 B_1^6\right.\\
   &\qquad\qquad\qquad~~\left.+29104 B_2 B_3^5 B_4^5 B_5^{10} B_1^3+1500 B_3^6 B_4^6 B_5^{12}\right)\\
   &-\dots,
    \end{split}}
\end{equation}
\begin{equation}
    {\tiny \begin{split}
        u_0(k)=&1+\frac{2B_1 B_2^3 \left(B_2 B_1^3+4 B_3 B_4 B_5^2\right)}{k^2}+\frac{6 B_2^4 B_3 B_4 B_5^2 \left(4 B_2 B_1^3+B_3 B_4 B_5^2\right)}{k^3}+\frac{6 B_1^2 B_2^6 \left(B_2^2 B_1^6+16 B_2 B_3 B_4 B_5^2 B_1^3+28 B_3^2 B_4^2 B_5^4\right)}{k^4}\\
        &+\frac{120 B_1
   B_2^7 B_3 B_4 B_5^2 \left(2 B_2^2 B_1^6+9 B_2 B_3 B_4 B_5^2 B_1^3+2 B_3^2 B_4^2 B_5^4\right)}{k^5}\\
   &+\frac{15 B_2^8 \left(2 B_2^4 B_1^{12}+72 B_2^3 B_3 B_4 B_5^2 B_1^9+540 B_2^2 B_3^2 B_4^2 B_5^4 B_1^6+512 B_2 B_3^3 B_4^3 B_5^6 B_1^3+9 B_3^4 B_4^4
   B_5^8\right)}{k^6}\\
   &+\frac{420 B_1^2 B_2^{10} B_3 B_4 B_5^2 \left(4 B_2^3 B_1^9+51 B_2^2 B_3 B_4 B_5^2 B_1^6+108 B_2 B_3^2 B_4^2 B_5^4 B_1^3+22 B_3^3 B_4^3 B_5^6\right)}{k^7}\\
   &+\frac{70 B_1 B_2^{11} \left(B_2^5 B_1^{15}+64 B_2^4 B_3 B_4 B_5^2 B_1^{12}+1104
   B_2^3 B_3^2 B_4^2 B_5^4 B_1^9+4096 B_2^2 B_3^3 B_4^3 B_5^6 B_1^6+2644 B_2 B_3^4 B_4^4 B_5^8 B_1^3+96 B_3^5 B_4^5 B_5^{10}\right)}{k^8}\\
        &+\frac{1680 B_2^{12} B_3 B_4 B_5^2 \left(6 B_2^5 B_1^{15}+150 B_2^4 B_3 B_4 B_5^2 B_1^{12}+868 B_2^3 B_3^2 B_4^2 B_5^4
   B_1^9+1158 B_2^2 B_3^3 B_4^3 B_5^6 B_1^6+222 B_2 B_3^4 B_4^4 B_5^8 B_1^3+B_3^5 B_4^5 B_5^{10}\right)}{k^9}\\
   &+\frac{252 B_1^2 B_2^{14}}{k^{10}} \left(B_2^6 B_1^{18}+100 B_2^5 B_3 B_4 B_5^2 B_1^{15}+3100 B_2^4 B_3^2 B_4^2 B_5^4 B_1^{12}+25600 B_2^3 B_3^3 B_4^3
   B_5^6 B_1^9+58150 B_2^2 B_3^4 B_4^4 B_5^8 B_1^6\right.\\
   &\qquad\qquad\qquad~~\left.+29104 B_2 B_3^5 B_4^5 B_5^{10} B_1^3+1500 B_3^6 B_4^6 B_5^{12}\right)\\
   &+\dots,
    \end{split}}
\end{equation}
for $k\geq p(1,1)\approx2.87752$, and when $k=k_\text{iso}$,
\begin{equation}
    \begin{split}
        m(P)=&-\frac{i(4\text{Li}_2(\text{e}^{b_1})+4\text{Li}_2(\text{e}^{b_2})+2\text{Li}_2(\text{e}^{b_3})+\text{Li}_2(\text{e}^{b_4})+4\text{Li}_2(\text{e}^{b_5})}{2\pi}\\
        &+\frac{1}{8}(i\pi\mathfrak{b}_0+2(-16\log(2)+8b_1\log(2\sin(\pi\mathfrak{b}_1))+8b_2\log(2\sin(\pi\mathfrak{b}_2))+4b_3\log(2\sin(\pi\mathfrak{b}_3))\\
        &+2b_4\log(2\sin(\pi a_3))+8b_5\log(2\sin(\pi\mathfrak{b}_5)))\\
        \approx&0.831627,
    \end{split}
\end{equation}
where
\begin{equation}
    \begin{split}
        &\mathfrak{b}_0\approx-1.426\text{ is a root of }3x^3-350194x^2+4114532x+6576872=0;\\
        &\mathfrak{b}_1\approx0.213\text{ is a root of }3x^3-170x^2-6x+9=0;\\
        &\mathfrak{b}_2\approx0.362\text{ is a root of }3x^3-67x^2+57x-12=0;\\
        &\mathfrak{b}_3\approx0.149\text{ is a root of }3x^3+103x^2-96x+12=0;\\
        &\mathfrak{b}_5\approx0.275\text{ is a root of }3x^3+125x^2-31x-1=0;
    \end{split}
\end{equation}
\paragraph{7. $\mathbb{C}^3/\mathbb{Z}_6$ $(1,2,3)$:}
\begin{equation}
    P=-z^2w^{-1}-z^{-1}w^{-1}-z^{-1}w-2z^{-1}-3w^{-1}-3zw^{-1}+k,
\end{equation}
with $k\geq k_\text{iso}=6$;
\begin{equation}
    m(P)=\log k-\frac{3}{k^2}-\frac{4}{k^3}-\frac{45}{2k^4}-\frac{72}{k^5}-\frac{340}{k^6}-\frac{1440}{k^7}-\frac{27405}{4k^8}-\frac{96880}{3k^9}-\frac{794178}{5k^{10}}-\dots,
\end{equation}
\begin{equation}
    u_0(k)=1+\frac{6}{k^2}+\frac{12}{k^3}+\frac{90}{k^4}+\frac{360}{k^5}+\frac{2040}{k^6}+\frac{10080}{k^7}+\frac{54810}{k^8}+\frac{290640}{k^9}+\frac{1588356}{k^{10}}+\dots
\end{equation}
for $k\geq p(1,1)=11$, and when $k=k_\text{iso}=6$,
\begin{equation}
    m(P)=-\frac{i\left(\pi^2+18\text{Li}_2\left(\frac{-1+i\sqrt{3}}{2}\right)\right)}{2\pi}\approx1.93840;
\end{equation}
\paragraph{8. SPP$/\mathbb{Z}_2$ $(0,1,1,1)$:}
\begin{equation}
    P=-\frac{C_1}{C_2C_3}(z+z^{-1}w^2+2w)-\frac{C_2C_3}{C_1}(w^{-1}+z^{-1})-2z^{-1}w+k,
\end{equation}
with $k\geq k_\text{iso}=6$, where
\begin{equation}
    C_1=\sin^2\left(\frac{\pi}{2\sqrt{3}}\right),C_2=\sin\left(\left(1-\frac{1}{\sqrt{3}}\right)\pi\right),C_3=\sin\left(\frac{1}{2}\left(1-\frac{1}{\sqrt{3}}\right)\pi\right);
\end{equation}
\begin{equation}
    m(P)=\log k-\frac{3}{k^2}-\frac{4}{k^3}-\frac{45}{2k^4}-\frac{72}{k^5}-\frac{340}{k^6}-\frac{1440}{k^7}-\frac{27405}{4k^8}-\frac{96880}{3k^9}-\frac{794178}{5k^{10}}-\dots,
\end{equation}
\begin{equation}
    u_0(k)=1+\frac{6}{k^2}+\frac{12}{k^3}+\frac{90}{k^4}+\frac{360}{k^5}+\frac{2040}{k^6}+\frac{10080}{k^7}+\frac{54810}{k^8}+\frac{290640}{k^9}+\frac{1588356}{k^{10}}+\dots
\end{equation}
for $k\geq p(1,1)\approx8.07697$, and when $k=k_\text{iso}=6$,
\begin{equation}
    \begin{split}
        m(P)=&-\frac{5}{6}i(3-2\sqrt{3})\pi+\log(2)+\log\left(\cos^2\left(\frac{\pi}{2\sqrt{3}}\right)\csc\left(\frac{\pi}{2\sqrt{3}}\right)\right)\\
        &+\frac{2}{\sqrt{3}}\log\left(2\csc^2\left(\frac{\pi}{\sqrt{3}}\right)\sin^3\left(\frac{\pi}{2\sqrt{3}}\right)\right)-\frac{2i\left(3\text{Li}_2(\text{e}^{i\pi/\sqrt{3}})+\text{Li}_2(\text{e}^{-2i\pi/\sqrt{3}})\right)}{\pi}\\
        \approx&1.77952;
    \end{split}
\end{equation}
\paragraph{9. PdP$_{3b}$:}
\begin{equation}
    P=-D_1^2D_2^2(z+z^{-1}w^{-1}+z^{-1}w+2z^{-1})-D_1^3D_3(w^{-1}+w)+k,
\end{equation}
with $k\geq k_\text{iso}=2D_1^3D_3+4D_1^2D_2^2\approx2.30196$, where
\begin{equation}
    D_1=\sin\left(\frac{3-\sqrt{5}}{2}\pi\right),D_2=\sin\left((-2+\sqrt{5})\pi\right),D_3=\sin\left(\frac{7-3\sqrt{5}}{2}\pi\right);
\end{equation}
\begin{equation}
    {\tiny \begin{split}
        m(P)=&\log k-\frac{2 D_3^2 D_1^6+4 D_2^4 D_1^4}{2 k^2}-\frac{4 D_1^7 D_2^4 D_3}{k^3}-\frac{6 D_3^4 D_1^{12}+48 D_2^4 D_3^2 D_1^{10}+36 D_2^8 D_1^8}{4 k^4}-\frac{120 D_2^4 D_3^3 D_1^{13}+240 D_2^8 D_3 D_1^{11}}{5 k^5}\\
        &-\frac{20 D_3^6 D_1^{18}+360 D_2^4 D_3^4
   D_1^{16}+1260 D_2^8 D_3^2 D_1^{14}+400 D_2^{12} D_1^{12}}{6 k^6}-\frac{840 D_2^4 D_3^5 D_1^{19}+5040 D_2^8 D_3^3 D_1^{17}+4200 D_2^{12} D_3 D_1^{15}}{7 k^7}\\
   &-\frac{70 D_3^8 D_1^{24}+2240 D_2^4 D_3^6 D_1^{22}+18480 D_2^8 D_3^4 D_1^{20}+29120 D_2^{12} D_3^2
   D_1^{18}+4900 D_2^{16} D_1^{16}}{8 k^8}\\
   &-\frac{5040 D_2^4 D_3^7 D_1^{25}+60480 D_2^8 D_3^5 D_1^{23}+154560 D_2^{12} D_3^3 D_1^{21}+70560 D_2^{16} D_3 D_1^{19}}{9 k^9}\\
   &-\frac{252 D_3^{10} D_1^{30}+12600 D_2^4 D_3^8 D_1^{28}+189000 D_2^8 D_3^6
   D_1^{26}+705600 D_2^{12} D_3^4 D_1^{24}+617400 D_2^{16} D_3^2 D_1^{22}+63504 D_2^{20} D_1^{20}}{10 k^{10}}-\dots,
    \end{split}}
\end{equation}
\begin{equation}
    {\tiny \begin{split}
        u_0(k)=&1+\frac{2 D_3^2 D_1^6+4 D_2^4 D_1^4}{k^2}+\frac{12 D_1^7 D_2^4 D_3}{k^3}+\frac{6 D_3^4 D_1^{12}+48 D_2^4 D_3^2 D_1^{10}+36 D_2^8 D_1^8}{k^4}+\frac{120 D_2^4 D_3^3 D_1^{13}+240 D_2^8 D_3 D_1^{11}}{k^5}\\
        &+\frac{20 D_3^6 D_1^{18}+360 D_2^4 D_3^4
   D_1^{16}+1260 D_2^8 D_3^2 D_1^{14}+400 D_2^{12} D_1^{12}}{k^6}+\frac{840 D_2^4 D_3^5 D_1^{19}+5040 D_2^8 D_3^3 D_1^{17}+4200 D_2^{12} D_3 D_1^{15}}{k^7}\\
   &+\frac{70 D_3^8 D_1^{24}+2240 D_2^4 D_3^6 D_1^{22}+18480 D_2^8 D_3^4 D_1^{20}+29120 D_2^{12} D_3^2
   D_1^{18}+4900 D_2^{16} D_1^{16}}{k^8}\\
   &+\frac{5040 D_2^4 D_3^7 D_1^{25}+60480 D_2^8 D_3^5 D_1^{23}+154560 D_2^{12} D_3^3 D_1^{21}+70560 D_2^{16} D_3 D_1^{19}}{k^9}\\
   &+\frac{252 D_3^{10} D_1^{30}+12600 D_2^4 D_3^8 D_1^{28}+189000 D_2^8 D_3^6
   D_1^{26}+705600 D_2^{12} D_3^4 D_1^{24}+617400 D_2^{16} D_3^2 D_1^{22}+63504 D_2^{20} D_1^{20}}{k^{10}}-\dots,
    \end{split}}
\end{equation}
for $k\geq p(1,1)\approx2.69833$, and when $k=k_\text{iso}$,
\begin{equation}
    \begin{split}
        m(P)=&\frac{361-162\sqrt{5}}{6}i\pi+9\log\left(\cos\left(\frac{\sqrt{5}\pi}{2}\right)\right)+7\log\left(\cos\left(\frac{3\sqrt{5}\pi}{2}\right)\right)+12\log(\csc(\sqrt{5}\pi))\\
        &+3\sqrt{5}\log\left(\sec\left(\frac{\sqrt{5}\pi}{2}\right)\sec\left(\frac{3\sqrt{5}\pi}{2}\right)\sin^2\left(\sqrt{5}\pi\right)\right)\\
        &-\frac{i\left(3\text{Li}_2(-\text{e}^{-i\sqrt{5}\pi})+3\text{Li}_2(\text{e}^{2i\sqrt{5}\pi})+\text{Li}_2(-\text{e}^{-3i\sqrt{5}\pi})\right)}{\pi}\\
        \approx&0.741874;
    \end{split}
\end{equation}
\paragraph{10. dP$_3$:}
\begin{equation}
    P=-z-zw^{-1}-w^{-1}-z^{-1}-z^{-1}w-w+k,
\end{equation}
with $k\geq k_\text{iso}=6$;
\begin{equation}
    m(P)=\log k-\frac{3}{k^2}-\frac{4}{k^3}-\frac{45}{2k^4}-\frac{72}{k^5}-\frac{340}{k^6}-\frac{1440}{k^7}-\frac{27405}{4k^8}-\frac{96880}{3k^9}-\frac{794178}{5k^{10}}-\dots,
\end{equation}
\begin{equation}
    u_0(k)=1+\frac{6}{k^2}+\frac{12}{k^3}+\frac{90}{k^4}+\frac{360}{k^5}+\frac{2040}{k^6}+\frac{10080}{k^7}+\frac{54810}{k^8}+\frac{290640}{k^9}+\frac{1588356}{k^{10}}+\dots
\end{equation}
for $k\geq p(1,1)=6$, and when $k=k_\text{iso}=6$,
\begin{equation}
    m(P)=-\frac{i\left(\pi^2+36\text{Li}_2\left(\frac{-1+i\sqrt{3}}{2}\right)+36\text{Li}_2\left(\frac{1+i\sqrt{3}}{2}\right)\right)}{12\pi}\approx1.61533;
\end{equation}
\paragraph{11. PdP$_2$:}
\begin{equation}
    P=-E_1^3E_2z-E_2E_3^2E_4w^{-1}-E_3^2E_5^2z^{-1}w^{-1}-E_6^4z^{-1}w-2E_3E_5E_6^2z^{-1}+k,
\end{equation}
with $k\geq k_\text{iso}=2E_1E_2E_3E_6+2E_1^2E_5E_6+E_1E_4E_6^2\approx2.17587$, where $E_i=\sin(\pi e_i/2)$ and
\begin{equation}
    \begin{split}
        &e_1\approx0.570\text{ is a root of }9x^4-78x^3+112x^2+16x-32=0;\\
        &e_2\approx0.876\text{ is a root of }27x^4-108x^3-96x^2+368x-192=0;\\
        &e_3\approx0.808\text{ is a root of }27x^4-108x^3+84x^2+28x-32=0;\\
        &e_4\approx0.306\text{ is a root of }27x^4+126x^3-864x^2+1088x-256=0;\\
        &e_5\approx0.502\text{ is a root of }9x^4-26x^3+4x^2+52x-24=0;\\
        &e_6\approx0.622\text{ is a root of }27x^4+126x^3+36x^2-52x-16=0;
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        m(P)=&\log k-\frac{2 E_1^3 E_2 E_3 E_5 E_6^2}{k^2}-\frac{2 E_1^3 E_2^2 E_3^2 E_4 E_6^4}{k^3}-\frac{9 E_1^6 E_2^2 E_3^2 E_5^2
   E_6^4}{k^4}-\frac{24 E_1^6 E_2^3 E_3^3 E_4 E_5 E_6^6}{k^5}\\
        &-\frac{400 E_2^3 E_3^3 E_5^3 E_6^6 E_1^9+90 E_2^4 E_3^4 E_4^2 E_6^8
   E_1^6}{6 k^6}-\frac{300 E_1^9 E_2^4 E_3^4 E_4 E_5^2 E_6^8}{k^7}\\
        &-\frac{4900 E_2^4 E_3^4 E_5^4 E_6^8 E_1^{12}+3360 E_2^5 E_3^5 E_4^2
   E_5 E_6^{10} E_1^9}{8 k^8}\\
   &-\frac{35280 E_2^5 E_3^5 E_4 E_5^3 E_6^{10} E_1^{12}+1680 E_2^6 E_3^6 E_4^3 E_6^{12} E_1^9}{9 k^9}\\
        &-\frac{63504
   E_2^5 E_3^5 E_5^5 E_6^{10} E_1^{15}+88200 E_2^6 E_3^6 E_4^2 E_5^2 E_6^{12} E_1^{12}}{10 k^{10}}-\dots,
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        u_0(k)=&1+\frac{4 E_1^3 E_2 E_3 E_5 E_6^2}{k^2}+\frac{6 E_1^3 E_2^2 E_3^2 E_4 E_6^4}{k^3}+\frac{36 E_1^6 E_2^2 E_3^2 E_5^2
   E_6^4}{k^4}+\frac{120 E_1^6 E_2^3 E_3^3 E_4 E_5 E_6^6}{k^5}\\
        &+\frac{400 E_2^3 E_3^3 E_5^3 E_6^6 E_1^9+90 E_2^4 E_3^4 E_4^2 E_6^8
   E_1^6}{k^6}+\frac{2100 E_1^9 E_2^4 E_3^4 E_4 E_5^2 E_6^8}{k^7}\\
        &+\frac{4900 E_2^4 E_3^4 E_5^4 E_6^8 E_1^{12}+3360 E_2^5 E_3^5 E_4^2
   E_5 E_6^{10} E_1^9}{k^8}\\
   &+\frac{35280 E_2^5 E_3^5 E_4 E_5^3 E_6^{10} E_1^{12}+1680 E_2^6 E_3^6 E_4^3 E_6^{12} E_1^9}{k^9}\\
        &+\frac{63504
   E_2^5 E_3^5 E_5^5 E_6^{10} E_1^{15}+88200 E_2^6 E_3^6 E_4^2 E_5^2 E_6^{12} E_1^{12}}{k^{10}}+\dots
    \end{split}
\end{equation}
for $k\geq p(1,1)\approx2.74127$, and when $k=k_\text{iso}$,
\begin{equation}
    {\tiny \begin{split}
        m(P)=&-\frac{i \left(3 \text{Li}_2\left(\text{e}^{i \pi  e_1}\right)+\text{Li}_2\left(\text{e}^{i \pi  e_2}\right)+2 \text{Li}_2\left(\text{e}^{i \pi  e_3}\right)+\text{Li}_2\left(\text{e}^{i \pi  e_4}\right)+2 \text{Li}_2\left(\text{e}^{i \pi  e_5}\right)+4 \text{Li}_2\left(\text{e}^{i \pi 
   e_6}\right)\right)}{2 \pi }\\
   &-\frac{1}{72} i \pi  \left(18 e_5^2+\mathfrak{e}_2^2+2 \mathfrak{e}_3^2+\mathfrak{e}_4^2+4 \mathfrak{e}_5^2+3 \mathfrak{e}_1^2-78\right)+\frac{1}{2} \left(3 e_1 \log \left(-i \text{e}^{\frac{1}{2} i \pi  e_1}\right)+e_2 \log \left(-i \text{e}^{\frac{1}{2} i \pi  e_2}\right)+2 e_3 \log
   \left(-i \text{e}^{\frac{1}{2} i \pi  e_3}\right)\right.\\
   &+e_4 \log \left(-i \text{e}^{\frac{1}{2} i \pi  e_4}\right)+2 e_5 \log \left(-i \text{e}^{\frac{1}{2} i \pi  e_5}\right)+4 e_6 \log \left(-i \text{e}^{\frac{1}{2} i \pi  e_6}\right)+3 e_1 \log \left(2 \sin \left(\frac{\pi e_1}{2}\right)\right)+e_2 \log \left(2 \sin \left(\frac{\pi  e_2}{2}\right)\right)\\
   &\left.+2 e_3 \log \left(2 \sin \left(\frac{\pi  e_3}{2}\right)\right)+e_4 \log \left(2 \sin \left(\frac{\pi  e_4}{2}\right)\right)+2 e_5 \log \left(2 \sin \left(\frac{\pi 
   e_5}{2}\right)\right)+4 e_6 \log \left(2 \sin \left(\frac{\pi  e_6}{2}\right)\right)-8\log2\right)\\
   \approx0.716493&,
    \end{split}}
\end{equation}
where
\begin{equation}
    \begin{split}
        &\mathfrak{e}_1\approx1.719\text{ is a root of }x^4-26x^3+112x^2+48x-288=0;\\
        &\mathfrak{e}_2\approx2.683\text{ is a root of }x^4-12x^3-32x^2+368x-576=0;\\
        &\mathfrak{e}_3\approx2.424\text{ is a root of }x^4-12x^3+28x^2+28x-96=0;\\
        &\mathfrak{e}_4\approx0.919\text{ is a root of }x^4+14x^3-288x^2+1088x-768=0;\\
        &\mathfrak{e}_5\approx1.867\text{ is a root of }x^4+14x^3+12x^2-52x-48=0;\\
    \end{split}
\end{equation}
\paragraph{12. dP$_2$:}
\begin{equation}
    P=-F_1F_2^2(z+w)-F_1F_3F_4(z^{-1}+w^{-1})-F_4^2F_5z^{-1}w^{-1}+k,
\end{equation}
with $k\geq k_\text{iso}=2F_1F_2(F_3+F_4)+F_2^2F_5\approx2.09211$, where
\begin{equation}
    \begin{split}
        &F_1=\sin\left(\frac{9-\sqrt{33}}{8}\pi\right),F_2=\sin\left(\frac{-21+5\sqrt{33}}{32}\pi\right),F_3=\sin\left(\frac{57-9\sqrt{33}}{32}\pi\right),\\
        &F_4=\sin\left(\frac{17-\sqrt{33}}{32}\pi\right),F_5=\sin\left(\frac{-5+\sqrt{33}}{4}\pi\right);
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        m(P)=&\log k-\frac{2F_1^2F_2^2F_3F_4}{k^2}-\frac{2F_1^2F_2^4F_4^2F_5}{k^3}-\frac{9F_1^4F_2^4F_3^2F_4^2}{k^4}-\frac{24F_1^4F_2^6F_3F_4^3F_5}{k^5}\\
        &-\frac{400F_1^6F_2^6F_3^3F_4^3+90F_1^4F_2^8F_4^4F_5^2}{6k^6}-\frac{300F_1^6F_2^8F_3^2F_4^4F_5}{k^7}\\
        &-\frac{4900F_1^8F_2^8F_3^4F_4^4+3360F_1^6F_2^{10}F_3F_4^5F_5^2}{8k^8}-\frac{35280F_1^8F_2^{10}F_3^3F_4^5F_5+1680F_1^6F_2^{12}F_4^6F_5^3}{9k^9}\\
        &-\frac{63504F_1^{10}F_2^{10}F_3^5F_4^5+88200F_1^8F_2{12}F_3^2F_4^6F_5^2}{10k^{10}}-\dots,
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        u_0(k)=&1+\frac{4F_1^2F_2^2F_3F_4}{k^2}+\frac{6F_1^2F_2^4F_4^2F_5}{k^3}+\frac{36F_1^4F_2^4F_3^2F_4^2}{k^4}+\frac{120F_1^4F_2^6F_3F_4^3F_5}{k^5}\\
        &+\frac{400F_1^6F_2^6F_3^3F_4^3+90F_1^4F_2^8F_4^4F_5^2}{k^6}+\frac{2100F_1^6F_2^8F_3^2F_4^4F_5}{k^7}\\
        &+\frac{4900F_1^8F_2^8F_3^4F_4^4+3360F_1^6F_2^{10}F_3F_4^5F_5^2}{k^8}+\frac{35280F_1^8F_2^{10}F_3^3F_4^5F_5+1680F_1^6F_2^{12}F_4^6F_5^3}{k^9}\\
        &+\frac{63504F_1^{10}F_2^{10}F_3^5F_4^5+88200F_1^8F_2{12}F_3^2F_4^6F_5^2}{k^{10}}+\dots
    \end{split}
\end{equation}
for $k\geq p(1,1)\approx2.19666$, and when $k=k_\text{iso}$,
\begin{equation}
    {\tiny \begin{split}
        m(P)=&\frac{1}{384 \pi }\left(-192 i \left(2 \text{Li}_2\left(\text{e}^{\frac{1}{16} i \left(57-9 \sqrt{33}\right) \pi }\right)+2 \text{Li}_2\left(\text{e}^{-\frac{1}{16} i \left(-17+\sqrt{33}\right) \pi }\right)+2 \text{Li}_2\left(\text{e}^{-\frac{1}{4} i
   \left(-9+\sqrt{33}\right) \pi }\right)+\text{Li}_2\left(\text{e}^{\frac{1}{2} i \left(-5+\sqrt{33}\right) \pi }\right)\right.\right.\\
   &\left.+4 \text{Li}_2\left(\text{e}^{\frac{1}{16} i \left(-21+5 \sqrt{33}\right) \pi }\right)\right)-24 \pi  \left(\left(\sqrt{33}-17\right)
   \log \left(\sqrt[32]{-1} \text{e}^{-\frac{1}{32} i \sqrt{33} \pi }\right)+4 \sqrt{33} \log \left((-1)^{5/8} \text{e}^{-\frac{1}{8} i \sqrt{33} \pi }\right)\right.\\
   &\left.-36 \log \left((-1)^{5/8} \text{e}^{-\frac{1}{8} i \sqrt{33} \pi }\right)-10 \sqrt{33} \log
   \left((-1)^{27/32} \text{e}^{\frac{5}{32} i \sqrt{33} \pi }\right)+42 \log \left((-1)^{27/32} \text{e}^{\frac{5}{32} i \sqrt{33} \pi }\right)-4 \sqrt{33} \log \left(\sqrt[4]{-1} \text{e}^{\frac{1}{4} i \sqrt{33} \pi }\right)\right.\\
   &\left.\left.+20 \log \left(\sqrt[4]{-1}
   \text{e}^{\frac{1}{4} i \sqrt{33} \pi }\right)+9 \sqrt{33} \log \left(-(-1)^{9/32} \text{e}^{-\frac{9}{32} i \sqrt{33} \pi }\right)-57 \log \left(-(-1)^{9/32} \text{e}^{-\frac{9}{32} i \sqrt{33} \pi }\right)+16 \log (8)\right.\right.\\
   &\left.\left.-10 \sqrt{33} \log \left(2 \sin
   \left(\frac{1}{32} \left(5 \sqrt{33}-21\right) \pi \right)\right)+42 \log \left(2 \sin \left(\frac{1}{32} \left(5 \sqrt{33}-21\right) \pi \right)\right)-4 \sqrt{33} \log \left(2 \sin \left(\frac{1}{4} \left(\sqrt{33}-5\right) \pi \right)\right)\right.\right.\\
   &\left.\left.+20 \log
   \left(2 \sin \left(\frac{1}{4} \left(\sqrt{33}-5\right) \pi \right)\right)+9 \sqrt{33} \log \left(2 \sin \left(\frac{1}{32} \left(57-9 \sqrt{33}\right) \pi \right)\right)-57 \log \left(2 \sin \left(\frac{1}{32} \left(57-9 \sqrt{33}\right) \pi
   \right)\right)\right.\right.\\
   &\left.\left.+\sqrt{33} \log \left(2 \cos \left(\frac{1}{32} \left(\sqrt{33}-1\right) \pi \right)\right)-17 \log \left(2 \cos \left(\frac{1}{32} \left(\sqrt{33}-1\right) \pi \right)\right)+4 \sqrt{33} \log \left(2 \cos \left(\frac{1}{8}
   \left(\sqrt{33}-5\right) \pi \right)\right)\right.\right.\\
   &\left.\left.-36 \log \left(2 \cos \left(\frac{1}{8} \left(\sqrt{33}-5\right) \pi \right)\right)\right)+i \left(783 \sqrt{33}-4319\right) \pi ^2\right)\approx0.580972;
    \end{split}}
\end{equation}
\paragraph{13. $Y^{2,2}$:}
\begin{equation}
    P=-w-z^{-1}w^{-1}-zw^{-1}-2w^{-1}+k,
\end{equation}
with $k\geq k_\text{iso}=4$;
\begin{equation}
    m(P)=\log k-2k^{-2}{}_4F_3\left(1,1,\frac{3}{2},\frac{3}{2};2,2,2;16k^{-2}\right),
\end{equation}
\begin{equation}
    u_0(k)={}_2F_1\left(\frac{1}{2},\frac{1}{2};1;16k^{-2}\right)
\end{equation}
for $k\geq p(1,1)=5$, and when $k=k_\text{iso}$,
\begin{equation}
    m(P)=-\frac{i\left(\pi^2+18\text{Li}_2\left(\frac{-1+i\sqrt{3}}{2}\right)\right)}{3\pi}\approx1.29226;
\end{equation}
\paragraph{14. dP$_1$:}
\begin{equation}
    P=-G_1^2G_2(z+z^{-1}w^{-1})-G_2^2G_3w^{-1}-G_4^3w+k,
\end{equation}
with $k\geq k_\text{iso}=2G_1^2G_4+G_2^2G_4+G_3G_4^2\approx1.99993$, where
\begin{equation}
    \begin{split}
        &G_1=\sin\left(\frac{2}{3}(-4+\sqrt{13})\pi\right),G_2=\sin\left(\frac{1}{6}(-1+\sqrt{13})\pi\right),\\
        &G_3=\sin\left(\frac{1}{6}(-17+5\sqrt{13})\pi\right),G_4=\sin\left(\frac{1}{2}(-3+\sqrt{13})\pi\right);
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        m(P)=&\log k-\frac{G_2^2 G_3 G_4^3}{k^2}-\frac{2 G_1^4 G_2^2 G_4^3}{k^3}-\frac{3 G_2^4 G_3^2 G_4^6}{2 k^4}-\frac{12 G_1^4 G_2^4 G_3 G_4^6}{k^5}\\
        &-\frac{20 G_2^6 G_3^3 G_4^9+90 G_1^8 G_2^4 G_4^6}{6 k^6}-\frac{60 G_1^4 G_2^6 G_3^2 G_4^9}{k^7}-\frac{70 G_2^8 G_3^4
   G_4^{12}+1680 G_1^8 G_2^6 G_3 G_4^9}{8 k^8}\\
   &-\frac{1680 G_2^6 G_4^9 G_1^{12}+2520 G_2^8 G_3^3 G_4^{12} G_1^4}{9 k^9}-\frac{252 G_2^{10} G_3^5 G_4^{15}+18900 G_1^8 G_2^8 G_3^2 G_4^{12}}{10 k^{10}}-\dots,
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        u_0(k)=&1+\frac{2G_2^2 G_3 G_4^3}{k^2}+\frac{6 G_1^4 G_2^2 G_4^3}{k^3}+\frac{6 G_2^4 G_3^2 G_4^6}{k^4}+\frac{60 G_1^4 G_2^4 G_3 G_4^6}{k^5}\\
        &+\frac{20 G_2^6 G_3^3 G_4^9+90 G_1^8 G_2^4 G_4^6}{k^6}+\frac{420 G_1^4 G_2^6 G_3^2 G_4^9}{k^7}+\frac{70 G_2^8 G_3^4
   G_4^{12}+1680 G_1^8 G_2^6 G_3 G_4^9}{k^8}\\
   &+\frac{1680 G_2^6 G_4^9 G_1^{12}+2520 G_2^8 G_3^3 G_4^{12} G_1^4}{k^9}+\frac{252 G_2^{10} G_3^5 G_4^{15}+18900 G_1^8 G_2^8 G_3^2 G_4^{12}}{k^{10}}+\dots
    \end{split}
\end{equation}
for $k\geq p(1,1)\approx2.08895$, and when $k=k_\text{iso}$,
\begin{equation}
    {\tiny \begin{split}
        m(P)=&\frac{1}{18} \left(-\frac{9 i \left(2 \text{Li}_2\left(-(-1)^{2/3} \text{e}^{\frac{1}{3} i \sqrt{13} \pi }\right)+3 \text{Li}_2\left(-\text{e}^{i \sqrt{13} \pi }\right)+4 \text{Li}_2\left(-\sqrt[3]{-1} \text{e}^{-\frac{4}{3} i \sqrt{13} \pi
   }\right)+\text{Li}_2\left(\sqrt[3]{-1} \text{e}^{\frac{5}{3} i \sqrt{13} \pi }\right)\right)}{\pi }\right.\\
   &+i \left(761-212 \sqrt{13}\right) \pi +3 \left(64 \log \left(\sin \left(\frac{1}{3} \left(\pi +2 \sqrt{13} \pi \right)\right)\right)+9 \left(\sqrt{13}-3\right)
   \log \left(\cos \left(\frac{\sqrt{13} \pi }{2}\right)\right)\right.\\
   &\left.\left.+16 \sqrt{13} \log \left(\csc \left(\frac{1}{3} \left(\pi +2 \sqrt{13} \pi \right)\right)\right)+\sqrt{13} \log \left(-\sin ^5\left(\frac{1}{6} \left(\pi +5 \sqrt{13} \pi \right)\right)
   \cos ^2\left(\frac{1}{6} \left(2+\sqrt{13}\right) \pi \right)\right)\right.\right.\\
   &\left.\left.+\log \left(-\csc ^{17}\left(\frac{1}{6} \left(\pi +5 \sqrt{13} \pi \right)\right) \sec ^2\left(\frac{1}{6} \left(2+\sqrt{13}\right) \pi \right)\right)\right)\right)\approx0.543128;
    \end{split}}
\end{equation}
\paragraph{15. $\mathbb{F}_0$:}
\begin{equation}
    P=-z-w-z^{-1}-w^{-1}+k,
\end{equation}
with $k\geq k_\text{iso}=4$;
\begin{equation}
    m(P)=\log k-2k^{-2}{}_4F_3\left(1,1,\frac{3}{2},\frac{3}{2};2,2,2;16k^{-2}\right),
\end{equation}
\begin{equation}
    u_0(k)={}_2F_1\left(\frac{1}{2},\frac{1}{2};1;16k^{-2}\right)
\end{equation}
for $k\geq p(1,1)=4$, and when $k=k_\text{iso}$,
\begin{equation}
    m(P)=\frac{4\mathcal{K}}{\pi}\approx1.16624;
\end{equation}
\paragraph{16. dP$_0$:}
\begin{equation}
    P=-z-w-z^{-1}w^{-1}+k,
\end{equation}
with $k\geq k_\text{iso}=3$;
\begin{equation}
    m(P)=\log k-2k^{-3}{}_4F_3\left(1,1,\frac{4}{3},\frac{5}{3};2,2,2;27k^{-3}\right),
\end{equation}
\begin{equation}
    u_0(k)={}_2F_1\left(\frac{1}{3},\frac{2}{3};1;27k^{-3}\right)
\end{equation}
for $k\geq p(1,1)=3$, and when $k=k_\text{iso}$,
\begin{equation}
    m(P)=-\frac{i\left(\pi^2+18\text{Li}_2\left(\frac{-1+i\sqrt{3}}{2}\right)\right)}{4\pi}\approx0.969198;
\end{equation}

\section{Areas of Holes in the Large $k$ Limit}\label{Ahlist}
Here, we plot all the spines (in red) of the triangulated reflexive polygons (in black). Notice that we have omitted all the external semi-infinite lines in the spines. The Newton polynomials are given in Appendix \ref{mahlerlist}.
\\

\tikzset{every picture/.style={line width=0.75pt}} \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,838); %set diagram left start at 0, and has height of 838

%Shape: Grid [id:dp825242200168689] 
\draw  [draw opacity=0] (460.5,321.4) -- (540.5,321.4) -- (540.5,401.4) -- (460.5,401.4) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (480.5,321.4) -- (480.5,401.4)(500.5,321.4) -- (500.5,401.4)(520.5,321.4) -- (520.5,401.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (460.5,341.4) -- (540.5,341.4)(460.5,361.4) -- (540.5,361.4)(460.5,381.4) -- (540.5,381.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (460.5,321.4) -- (540.5,321.4) -- (540.5,401.4) -- (460.5,401.4) -- cycle ;
%Straight Lines [id:da5691958948699953] 
\draw [line width=1.5]    (500.5,341.4) -- (480.5,341.4) ;
%Shape: Grid [id:dp9536859795403847] 
\draw  [draw opacity=0] (160.5,321.5) -- (240.5,321.5) -- (240.5,401.5) -- (160.5,401.5) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (180.5,321.5) -- (180.5,401.5)(200.5,321.5) -- (200.5,401.5)(220.5,321.5) -- (220.5,401.5) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (160.5,341.5) -- (240.5,341.5)(160.5,361.5) -- (240.5,361.5)(160.5,381.5) -- (240.5,381.5) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (160.5,321.5) -- (240.5,321.5) -- (240.5,401.5) -- (160.5,401.5) -- cycle ;
%Straight Lines [id:da8232393759342878] 
\draw [line width=1.5]    (200.5,381.5) -- (180.5,361.5) ;
%Shape: Grid [id:dp9322548745628676] 
\draw  [draw opacity=0] (259.5,121.5) -- (339.5,121.5) -- (339.5,201.5) -- (259.5,201.5) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (279.5,121.5) -- (279.5,201.5)(299.5,121.5) -- (299.5,201.5)(319.5,121.5) -- (319.5,201.5) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (259.5,141.5) -- (339.5,141.5)(259.5,161.5) -- (339.5,161.5)(259.5,181.5) -- (339.5,181.5) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (259.5,121.5) -- (339.5,121.5) -- (339.5,201.5) -- (259.5,201.5) -- cycle ;
%Straight Lines [id:da9938782279905574] 
\draw [line width=1.5]    (299.5,161.5) -- (319.5,141.5) ;
%Straight Lines [id:da18152631809760944] 
\draw [line width=1.5]    (319.5,141.5) -- (279.5,141.5) ;
%Shape: Grid [id:dp35202859024349453] 
\draw  [draw opacity=0] (59,122) -- (139,122) -- (139,202) -- (59,202) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (79,122) -- (79,202)(99,122) -- (99,202)(119,122) -- (119,202) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (59,142) -- (139,142)(59,162) -- (139,162)(59,182) -- (139,182) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (59,122) -- (139,122) -- (139,202) -- (59,202) -- cycle ;
%Straight Lines [id:da12602211688242093] 
\draw [line width=1.5]    (139,182) -- (119,162) ;
%Straight Lines [id:da29078089811215757] 
\draw [line width=1.5]    (119,162) -- (59,182) ;
%Straight Lines [id:da6018232644014307] 
\draw [line width=1.5]    (139,142) -- (59,182) ;
%Straight Lines [id:da8427319540458731] 
\draw [line width=1.5]    (139,182) -- (139,142) ;
%Straight Lines [id:da6440677668533465] 
\draw [line width=1.5]    (119,162) -- (139,142) ;
%Straight Lines [id:da5827862719854084] 
\draw [line width=1.5]    (139,182) -- (59,182) ;
%Shape: Grid [id:dp9307832756013272] 
\draw  [draw opacity=0] (159.5,121.5) -- (239.5,121.5) -- (239.5,201.5) -- (159.5,201.5) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (179.5,121.5) -- (179.5,201.5)(199.5,121.5) -- (199.5,201.5)(219.5,121.5) -- (219.5,201.5) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (159.5,141.5) -- (239.5,141.5)(159.5,161.5) -- (239.5,161.5)(159.5,181.5) -- (239.5,181.5) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (159.5,121.5) -- (239.5,121.5) -- (239.5,201.5) -- (159.5,201.5) -- cycle ;
%Straight Lines [id:da2113198615423466] 
\draw [line width=1.5]    (159.5,181.5) -- (199.5,141.5) ;
%Straight Lines [id:da9058990775223685] 
\draw [line width=1.5]    (219.5,181.5) -- (159.5,181.5) ;
%Straight Lines [id:da4556474263466228] 
\draw [line width=1.5]    (219.5,181.5) -- (219.5,141.5) ;
%Straight Lines [id:da13093324880323043] 
\draw [line width=1.5]    (219.5,181.5) -- (199.5,161.5) ;
%Straight Lines [id:da9857672050030706] 
\draw [line width=1.5]    (159.5,181.5) -- (199.5,161.5) ;
%Straight Lines [id:da5397456101841291] 
\draw [line width=1.5]    (219.5,141.5) -- (199.5,161.5) ;
%Straight Lines [id:da3657447393244262] 
\draw [line width=1.5]    (279.5,181.5) -- (279.5,141.5) ;
%Straight Lines [id:da5396722821435345] 
\draw [line width=1.5]    (319.5,181.5) -- (279.5,181.5) ;
%Straight Lines [id:da4782521342428132] 
\draw [line width=1.5]    (319.5,181.5) -- (319.5,141.5) ;
%Straight Lines [id:da6082944180527345] 
\draw [line width=1.5]    (319.5,181.5) -- (299.5,161.5) ;
%Straight Lines [id:da1902522823724757] 
\draw [line width=1.5]    (299.5,161.5) -- (279.5,141.5) ;
%Straight Lines [id:da3053580397515048] 
\draw [line width=1.5]    (299.5,161.5) -- (279.5,181.5) ;
%Straight Lines [id:da5670507339044546] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (299.5,181.5) -- (319.5,161.5) ;
%Straight Lines [id:da8627003756977769] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (79,122) -- (119,162) ;
%Straight Lines [id:da4262025892905208] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (99,182) -- (119,162) ;
%Straight Lines [id:da43017747792463856] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (79,122) -- (99,182) ;
%Straight Lines [id:da20763668764455834] 
\draw [line width=1.5]    (219.5,141.5) -- (199.5,141.5) ;
%Straight Lines [id:da18814180174554052] 
\draw [line width=1.5]    (199.5,141.5) -- (199.5,161.5) ;
%Straight Lines [id:da09031562572850849] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (179.5,141.5) -- (199.5,141.5) ;
%Straight Lines [id:da15042361416328376] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (179.5,141.5) -- (199.5,181.5) ;
%Straight Lines [id:da8636260609414963] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (199.5,181.5) -- (219.5,161.5) ;
%Straight Lines [id:da5901015609198335] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (219.5,161.5) -- (199.5,141.5) ;
%Straight Lines [id:da6013444696470582] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (299.5,141.5) -- (319.5,161.5) ;
%Straight Lines [id:da5403946585881616] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (279.5,161.5) -- (299.5,141.5) ;
%Straight Lines [id:da08562002405221558] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (279.5,161.5) -- (299.5,181.5) ;
%Shape: Grid [id:dp8988256121989784] 
\draw  [draw opacity=0] (59,20.2) -- (139,20.2) -- (139,100.2) -- (59,100.2) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (79,20.2) -- (79,100.2)(99,20.2) -- (99,100.2)(119,20.2) -- (119,100.2) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (59,40.2) -- (139,40.2)(59,60.2) -- (139,60.2)(59,80.2) -- (139,80.2) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (59,20.2) -- (139,20.2) -- (139,100.2) -- (59,100.2) -- cycle ;
%Straight Lines [id:da2818077691259473] 
\draw [line width=1.5]    (139,80.2) -- (99,60.2) ;
%Straight Lines [id:da7803431050727274] 
\draw [line width=1.5]    (99,60.2) -- (79,80.2) ;
%Straight Lines [id:da8874563485443054] 
\draw [line width=1.5]    (139,80.2) -- (79,20.2) ;
%Straight Lines [id:da7552283879530357] 
\draw [line width=1.5]    (79,80.2) -- (79,20.2) ;
%Straight Lines [id:da5086259396406185] 
\draw [line width=1.5]    (99,60.2) -- (79,20.2) ;
%Straight Lines [id:da008471996190476672] 
\draw [line width=1.5]    (139,80.2) -- (79,80.2) ;
%Straight Lines [id:da580327589100782] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (79,60.2) -- (99,80.2) ;
%Straight Lines [id:da10686441575630878] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (79,60.2) -- (119,40.2) ;
%Straight Lines [id:da4171023243331866] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (119,40.2) -- (99,80.2) ;
%Shape: Grid [id:dp35209393430520564] 
\draw  [draw opacity=0] (360.5,222.4) -- (440.5,222.4) -- (440.5,302.4) -- (360.5,302.4) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (380.5,222.4) -- (380.5,302.4)(400.5,222.4) -- (400.5,302.4)(420.5,222.4) -- (420.5,302.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (360.5,242.4) -- (440.5,242.4)(360.5,262.4) -- (440.5,262.4)(360.5,282.4) -- (440.5,282.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (360.5,222.4) -- (440.5,222.4) -- (440.5,302.4) -- (360.5,302.4) -- cycle ;
%Straight Lines [id:da23680743822510397] 
\draw [line width=1.5]    (400.5,262.4) -- (400.5,282.4) ;
%Straight Lines [id:da5452154787175585] 
\draw [line width=1.5]    (400.5,282.4) -- (380.5,262.4) ;
%Straight Lines [id:da5760185713359078] 
\draw [line width=1.5]    (400.5,262.4) -- (420.5,262.4) ;
%Straight Lines [id:da6333640480623439] 
\draw [line width=1.5]    (420.5,262.4) -- (380.5,222.4) ;
%Shape: Grid [id:dp06014636075279922] 
\draw  [draw opacity=0] (161.5,221.4) -- (241.5,221.4) -- (241.5,301.4) -- (161.5,301.4) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (181.5,221.4) -- (181.5,301.4)(201.5,221.4) -- (201.5,301.4)(221.5,221.4) -- (221.5,301.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (161.5,241.4) -- (241.5,241.4)(161.5,261.4) -- (241.5,261.4)(161.5,281.4) -- (241.5,281.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (161.5,221.4) -- (241.5,221.4) -- (241.5,301.4) -- (161.5,301.4) -- cycle ;
%Straight Lines [id:da4453167762875698] 
\draw [line width=1.5]    (161.5,281.4) -- (201.5,241.4) ;
%Straight Lines [id:da08657174338470752] 
\draw [line width=1.5]    (221.5,281.4) -- (161.5,281.4) ;
%Straight Lines [id:da1720936634368535] 
\draw [line width=1.5]    (221.5,281.4) -- (221.5,261.4) ;
%Straight Lines [id:da1982400457346023] 
\draw [line width=1.5]    (221.5,281.4) -- (201.5,261.4) ;
%Straight Lines [id:da7669638222545982] 
\draw [line width=1.5]    (161.5,281.4) -- (201.5,261.4) ;
%Straight Lines [id:da961687684454211] 
\draw [line width=1.5]    (221.5,261.4) -- (201.5,261.4) ;
%Straight Lines [id:da8506402874572914] 
\draw [line width=1.5]    (380.5,262.4) -- (380.5,222.4) ;
%Straight Lines [id:da13494420678948416] 
\draw [line width=1.5]    (420.5,282.4) -- (400.5,282.4) ;
%Straight Lines [id:da10229013925693398] 
\draw [line width=1.5]    (420.5,282.4) -- (420.5,262.4) ;
%Straight Lines [id:da26572793565487585] 
\draw [line width=1.5]    (420.5,282.4) -- (400.5,262.4) ;
%Straight Lines [id:da02817098476049673] 
\draw [line width=1.5]    (400.5,262.4) -- (380.5,222.4) ;
%Straight Lines [id:da38207878311962107] 
\draw [line width=1.5]    (400.5,262.4) -- (380.5,262.4) ;
%Straight Lines [id:da12837346601194932] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (400.5,282.4) -- (420.5,262.4) ;
%Straight Lines [id:da20788872052616258] 
\draw [line width=1.5]    (221.5,261.4) -- (201.5,241.4) ;
%Straight Lines [id:da38728373812074834] 
\draw [line width=1.5]    (201.5,241.4) -- (201.5,261.4) ;
%Straight Lines [id:da7094568439500695] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (181.5,241.4) -- (221.5,241.4) ;
%Straight Lines [id:da0026322867811456874] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (181.5,241.4) -- (201.5,281.4) ;
%Straight Lines [id:da6220287280437449] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (201.5,281.4) -- (221.5,261.4) ;
%Straight Lines [id:da9921222191373078] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (221.5,261.4) -- (221.5,241.4) ;
%Straight Lines [id:da06538110341738812] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (420.5,242.4) -- (420.5,262.4) ;
%Straight Lines [id:da2653737881493601] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (380.5,262.4) -- (420.5,242.4) ;
%Straight Lines [id:da6379400417271901] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (380.5,282.4) -- (400.5,282.4) ;
%Straight Lines [id:da2887829138532936] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (380.5,262.4) -- (380.5,282.4) ;
%Shape: Grid [id:dp16252203402877496] 
\draw  [draw opacity=0] (60,322) -- (140,322) -- (140,402) -- (60,402) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (80,322) -- (80,402)(100,322) -- (100,402)(120,322) -- (120,402) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (60,342) -- (140,342)(60,362) -- (140,362)(60,382) -- (140,382) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (60,322) -- (140,322) -- (140,402) -- (60,402) -- cycle ;
%Straight Lines [id:da7331075635891062] 
\draw [line width=1.5]    (140,382) -- (100,362) ;
%Straight Lines [id:da8042149990044807] 
\draw [line width=1.5]    (100,362) -- (80,382) ;
%Straight Lines [id:da08105747520666706] 
\draw [line width=1.5]    (140,382) -- (80,342) ;
%Straight Lines [id:da46397992218801454] 
\draw [line width=1.5]    (80,382) -- (80,342) ;
%Straight Lines [id:da09567135315335262] 
\draw [line width=1.5]    (100,362) -- (80,342) ;
%Straight Lines [id:da3380050921064033] 
\draw [line width=1.5]    (140,382) -- (80,382) ;
%Straight Lines [id:da6994747892081881] 
\draw [line width=1.5]    (180.5,361.5) -- (180.5,321.5) ;
%Straight Lines [id:da9241269434127368] 
\draw [line width=1.5]    (200.5,361.5) -- (180.5,361.5) ;
%Straight Lines [id:da1980547221333766] 
\draw [line width=1.5]    (200.5,381.5) -- (220.5,361.5) ;
%Straight Lines [id:da32292789804918365] 
\draw [line width=1.5]    (200.5,361.5) -- (180.5,321.5) ;
%Straight Lines [id:da6499306887730705] 
\draw [line width=1.5]    (200.5,381.5) -- (200.5,361.5) ;
%Straight Lines [id:da9242493027438521] 
\draw [line width=1.5]    (220.5,361.5) ;
%Straight Lines [id:da5123529181945188] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (80,362) -- (120,322) ;
%Straight Lines [id:da12518993753167784] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (100,382) -- (120,322) ;
%Straight Lines [id:da8367002555538681] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (80,362) -- (100,382) ;
%Straight Lines [id:da05893122831895892] 
\draw [line width=1.5]    (220.5,361.5) -- (180.5,321.5) ;
%Straight Lines [id:da6467793568533113] 
\draw [line width=1.5]    (200.5,361.5) -- (220.5,361.5) ;
%Straight Lines [id:da7623381949430341] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (180.5,361.5) -- (220.5,341.5) ;
%Straight Lines [id:da07311367279570957] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (180.5,361.5) -- (180.5,381.5) ;
%Straight Lines [id:da6614616479690718] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (180.5,381.5) -- (220.5,381.5) ;
%Straight Lines [id:da43138955047067906] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (220.5,381.5) -- (220.5,341.5) ;
%Shape: Grid [id:dp5081096326520023] 
\draw  [draw opacity=0] (360.5,320.4) -- (440.5,320.4) -- (440.5,400.4) -- (360.5,400.4) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (380.5,320.4) -- (380.5,400.4)(400.5,320.4) -- (400.5,400.4)(420.5,320.4) -- (420.5,400.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (360.5,340.4) -- (440.5,340.4)(360.5,360.4) -- (440.5,360.4)(360.5,380.4) -- (440.5,380.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (360.5,320.4) -- (440.5,320.4) -- (440.5,400.4) -- (360.5,400.4) -- cycle ;
%Straight Lines [id:da38141380575512174] 
\draw [line width=1.5]    (400.5,360.4) -- (400.5,380.4) ;
%Straight Lines [id:da49749676493866235] 
\draw [line width=1.5]    (400.5,340.4) -- (380.5,340.4) ;
%Straight Lines [id:da94636213455573] 
\draw [line width=1.5]    (400.5,360.4) -- (420.5,360.4) ;
%Straight Lines [id:da1881928132827011] 
\draw [line width=1.5]    (420.5,360.4) -- (400.5,340.4) ;
%Straight Lines [id:da005888791711428976] 
\draw [line width=1.5]    (380.5,380.4) -- (380.5,340.4) ;
%Straight Lines [id:da8675364180131733] 
\draw [line width=1.5]    (400.5,380.4) -- (380.5,380.4) ;
%Straight Lines [id:da6255379317810774] 
\draw [line width=1.5]    (400.5,380.4) -- (420.5,360.4) ;
%Straight Lines [id:da4669359967751632] 
\draw [line width=1.5]    (400.5,360.4) -- (400.5,340.4) ;
%Straight Lines [id:da5818860844525036] 
\draw [line width=1.5]    (400.5,360.4) -- (380.5,340.4) ;
%Straight Lines [id:da5777384567076773] 
\draw [line width=1.5]    (400.5,360.4) -- (380.5,380.4) ;
%Straight Lines [id:da9748732316769448] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (420.5,380.4) -- (420.5,340.4) ;
%Straight Lines [id:da8526549536166548] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (400.5,340.4) -- (420.5,340.4) ;
%Straight Lines [id:da05720736712810792] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (380.5,360.4) -- (400.5,340.4) ;
%Straight Lines [id:da9079724832303384] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (400.5,380.4) -- (420.5,380.4) ;
%Straight Lines [id:da5646461799498439] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (380.5,360.4) -- (400.5,380.4) ;
%Straight Lines [id:da8686109106704201] 
\draw [line width=1.5]    (500.5,361.4) -- (500.5,381.4) ;
%Straight Lines [id:da009634859585637257] 
\draw [line width=1.5]    (500.5,381.4) -- (480.5,361.4) ;
%Straight Lines [id:da06906507048636912] 
\draw [line width=1.5]    (500.5,361.4) -- (520.5,361.4) ;
%Straight Lines [id:da7139473730278008] 
\draw [line width=1.5]    (520.5,361.4) -- (500.5,341.4) ;
%Straight Lines [id:da004497128679901152] 
\draw [line width=1.5]    (480.5,361.4) -- (480.5,341.4) ;
%Straight Lines [id:da6818049072342642] 
\draw [line width=1.5]    (520.5,381.4) -- (500.5,381.4) ;
%Straight Lines [id:da19748122856625883] 
\draw [line width=1.5]    (520.5,381.4) -- (520.5,361.4) ;
%Straight Lines [id:da9946748477662606] 
\draw [line width=1.5]    (520.5,381.4) -- (500.5,361.4) ;
%Straight Lines [id:da9613982710060869] 
\draw [line width=1.5]    (500.5,361.4) -- (480.5,341.4) ;
%Straight Lines [id:da19064858204260293] 
\draw [line width=1.5]    (500.5,361.4) -- (480.5,361.4) ;
%Straight Lines [id:da030914939985851486] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (500.5,381.4) -- (520.5,361.4) ;
%Straight Lines [id:da07784515024618632] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (520.5,341.4) -- (520.5,361.4) ;
%Straight Lines [id:da09970319900013425] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (480.5,361.4) -- (500.5,341.4) ;
%Straight Lines [id:da7976170509849272] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (500.5,341.4) -- (520.5,341.4) ;
%Straight Lines [id:da5289003042579441] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (480.5,361.4) -- (480.5,381.4) ;
%Straight Lines [id:da8543945770394057] 
\draw [line width=1.5]    (520.5,381.4) -- (500.5,361.4) ;
%Straight Lines [id:da6565052524214909] 
\draw [line width=1.5]    (520.5,381.4) -- (500.5,361.4) ;
%Straight Lines [id:da8825416566683035] 
\draw [line width=1.5]    (520.5,381.4) -- (500.5,361.4) ;
%Straight Lines [id:da19583454096274044] 
\draw [line width=1.5]    (520.5,381.4) -- (500.5,361.4) ;
%Straight Lines [id:da0657068075499605] 
\draw [line width=1.5]    (500.5,361.4) -- (500.5,341.4) ;
%Straight Lines [id:da15923598488614754] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (480.5,381.4) -- (500.5,381.4) ;
%Shape: Grid [id:dp3255515505184432] 
\draw  [draw opacity=0] (360,420.4) -- (440,420.4) -- (440,500.4) -- (360,500.4) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (380,420.4) -- (380,500.4)(400,420.4) -- (400,500.4)(420,420.4) -- (420,500.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (360,440.4) -- (440,440.4)(360,460.4) -- (440,460.4)(360,480.4) -- (440,480.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (360,420.4) -- (440,420.4) -- (440,500.4) -- (360,500.4) -- cycle ;
%Straight Lines [id:da27604241777541283] 
\draw [line width=1.5]    (400,460.4) -- (400,480.4) ;
%Straight Lines [id:da6041877937130387] 
\draw [line width=1.5]    (400,460.4) -- (400,440.4) ;
%Straight Lines [id:da14266359457415612] 
\draw [line width=1.5]    (400,460.4) -- (420,460.4) ;
%Straight Lines [id:da3698407264967769] 
\draw [line width=1.5]    (400,440.4) -- (380,460.4) ;
%Shape: Grid [id:dp31951632159251186] 
\draw  [draw opacity=0] (159.5,420.4) -- (239.5,420.4) -- (239.5,500.4) -- (159.5,500.4) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (179.5,420.4) -- (179.5,500.4)(199.5,420.4) -- (199.5,500.4)(219.5,420.4) -- (219.5,500.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (159.5,440.4) -- (239.5,440.4)(159.5,460.4) -- (239.5,460.4)(159.5,480.4) -- (239.5,480.4) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (159.5,420.4) -- (239.5,420.4) -- (239.5,500.4) -- (159.5,500.4) -- cycle ;
%Straight Lines [id:da678462938772181] 
\draw [line width=1.5]    (179.5,480.4) -- (179.5,440.4) ;
%Straight Lines [id:da888034477455514] 
\draw [line width=1.5]    (199.5,480.4) -- (179.5,480.4) ;
%Straight Lines [id:da17260413003972253] 
\draw [line width=1.5]    (199.5,480.4) -- (219.5,460.4) ;
%Straight Lines [id:da5140912890836504] 
\draw [line width=1.5]    (199.5,480.4) -- (199.5,460.4) ;
%Straight Lines [id:da9897369532473377] 
\draw [line width=1.5]    (179.5,480.4) -- (199.5,460.4) ;
%Straight Lines [id:da8973119982730986] 
\draw [line width=1.5]    (219.5,460.4) -- (199.5,460.4) ;
%Straight Lines [id:da31292310773810983] 
\draw [line width=1.5]    (380,480.4) -- (380,460.4) ;
%Straight Lines [id:da01922059801476217] 
\draw [line width=1.5]    (400,480.4) -- (380,480.4) ;
%Straight Lines [id:da2786333590740897] 
\draw [line width=1.5]    (400,480.4) -- (420,460.4) ;
%Straight Lines [id:da09024027951634706] 
\draw [line width=1.5]    (380,480.4) -- (400,460.4) ;
%Straight Lines [id:da4268405721672719] 
\draw [line width=1.5]    (420,460.4) -- (400,440.4) ;
%Straight Lines [id:da25758698381393375] 
\draw [line width=1.5]    (400,460.4) -- (380,460.4) ;
%Straight Lines [id:da8896362177258197] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (400,480.4) -- (420,480.4) ;
%Straight Lines [id:da09742929378319709] 
\draw [line width=1.5]    (219.5,460.4) -- (179.5,440.4) ;
%Straight Lines [id:da6239094012251616] 
\draw [line width=1.5]    (179.5,440.4) -- (199.5,460.4) ;
%Straight Lines [id:da44225701583522636] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (179.5,460.4) -- (219.5,420.4) ;
%Straight Lines [id:da3325931388609371] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (179.5,460.4) -- (199.5,480.4) ;
%Straight Lines [id:da26720206460660223] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (199.5,480.4) -- (219.5,480.4) ;
%Straight Lines [id:da03577185814328243] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (219.5,480.4) -- (219.5,420.4) ;
%Straight Lines [id:da6701274992708306] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (420,440.4) -- (420,480.4) ;
%Straight Lines [id:da27584050792219217] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (400,480.4) -- (380,460.4) ;
%Straight Lines [id:da9691454270098254] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (380,440.4) -- (420,440.4) ;
%Straight Lines [id:da433200933218467] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (380,440.4) -- (380,460.4) ;
%Shape: Grid [id:dp7959692107542118] 
\draw  [draw opacity=0] (260,520.3) -- (340,520.3) -- (340,600.3) -- (260,600.3) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (280,520.3) -- (280,600.3)(300,520.3) -- (300,600.3)(320,520.3) -- (320,600.3) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (260,540.3) -- (340,540.3)(260,560.3) -- (340,560.3)(260,580.3) -- (340,580.3) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (260,520.3) -- (340,520.3) -- (340,600.3) -- (260,600.3) -- cycle ;
%Straight Lines [id:da8498147886465977] 
\draw [line width=1.5]    (300,560.3) -- (300,540.3) ;
%Straight Lines [id:da9509734964142633] 
\draw [line width=1.5]    (320,560.3) -- (300,540.3) ;
%Shape: Grid [id:dp9654565890518076] 
\draw  [draw opacity=0] (59.5,520.8) -- (139.5,520.8) -- (139.5,600.8) -- (59.5,600.8) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (79.5,520.8) -- (79.5,600.8)(99.5,520.8) -- (99.5,600.8)(119.5,520.8) -- (119.5,600.8) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (59.5,540.8) -- (139.5,540.8)(59.5,560.8) -- (139.5,560.8)(59.5,580.8) -- (139.5,580.8) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (59.5,520.8) -- (139.5,520.8) -- (139.5,600.8) -- (59.5,600.8) -- cycle ;
%Straight Lines [id:da7539270843181631] 
\draw [line width=1.5]    (119.5,580.8) -- (99.5,560.8) ;
%Straight Lines [id:da5915830886671238] 
\draw [line width=1.5]    (99.5,560.8) -- (79.5,580.8) ;
%Straight Lines [id:da004522006654621213] 
\draw [line width=1.5]    (99.5,540.8) -- (79.5,580.8) ;
%Straight Lines [id:da8644230715348749] 
\draw [line width=1.5]    (119.5,580.8) -- (99.5,540.8) ;
%Straight Lines [id:da7897851570992036] 
\draw [line width=1.5]    (99.5,560.8) -- (99.5,540.8) ;
%Straight Lines [id:da20467580994614898] 
\draw [line width=1.5]    (119.5,580.8) -- (79.5,580.8) ;
%Shape: Grid [id:dp15419930564043005] 
\draw  [draw opacity=0] (160,520.3) -- (240,520.3) -- (240,600.3) -- (160,600.3) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (180,520.3) -- (180,600.3)(200,520.3) -- (200,600.3)(220,520.3) -- (220,600.3) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (160,540.3) -- (240,540.3)(160,560.3) -- (240,560.3)(160,580.3) -- (240,580.3) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (160,520.3) -- (240,520.3) -- (240,600.3) -- (160,600.3) -- cycle ;
%Straight Lines [id:da3554910309641137] 
\draw [line width=1.5]    (180,580.3) -- (200,540.3) ;
%Straight Lines [id:da8011301390034586] 
\draw [line width=1.5]    (200,580.3) -- (180,580.3) ;
%Straight Lines [id:da7606406606186846] 
\draw [line width=1.5]    (200,580.3) -- (220,560.3) ;
%Straight Lines [id:da3293011616380468] 
\draw [line width=1.5]    (200,580.3) -- (200,560.3) ;
%Straight Lines [id:da5325672769146428] 
\draw [line width=1.5]    (180,580.3) -- (200,560.3) ;
%Straight Lines [id:da5266843264978864] 
\draw [line width=1.5]    (220,560.3) -- (200,560.3) ;
%Straight Lines [id:da8577774563270157] 
\draw [line width=1.5]    (280,560.3) -- (300,540.3) ;
%Straight Lines [id:da47814275656898353] 
\draw [line width=1.5]    (300,580.3) -- (280,560.3) ;
%Straight Lines [id:da6943293885835766] 
\draw [line width=1.5]    (300,580.3) -- (320,560.3) ;
%Straight Lines [id:da6159149810937166] 
\draw [line width=1.5]    (320,560.3) -- (300,560.3) ;
%Straight Lines [id:da5849995286291247] 
\draw [line width=1.5]    (300,560.3) -- (280,560.3) ;
%Straight Lines [id:da3387316907047153] 
\draw [line width=1.5]    (300,560.3) -- (300,580.3) ;
%Straight Lines [id:da33280889842750194] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (280,580.3) -- (320,580.3) ;
%Straight Lines [id:da08229436023622694] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (59.5,540.8) -- (139.5,540.8) ;
%Straight Lines [id:da912958256851216] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (99.5,580.8) -- (139.5,540.8) ;
%Straight Lines [id:da3893242552509055] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (59.5,540.8) -- (99.5,580.8) ;
%Straight Lines [id:da4951710649159098] 
\draw [line width=1.5]    (220,560.3) -- (200,540.3) ;
%Straight Lines [id:da4581261166286519] 
\draw [line width=1.5]    (200,540.3) -- (200,560.3) ;
%Straight Lines [id:da560625912818544] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (160,540.3) -- (220,540.3) ;
%Straight Lines [id:da3244308392278943] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (160,540.3) -- (200,580.3) ;
%Straight Lines [id:da7612155817180346] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (200,580.3) -- (220,580.3) ;
%Straight Lines [id:da10446316535798195] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (220,580.3) -- (220,540.3) ;
%Straight Lines [id:da5019630607600167] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (320,540.3) -- (320,580.3) ;
%Straight Lines [id:da7199042003873533] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (280,540.3) -- (320,540.3) ;
%Straight Lines [id:da3039020844873357] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (280,540.3) -- (280,580.3) ;
%Shape: Grid [id:dp06690192393849115] 
\draw  [draw opacity=0] (60,620.8) -- (140,620.8) -- (140,700.8) -- (60,700.8) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (80,620.8) -- (80,700.8)(100,620.8) -- (100,700.8)(120,620.8) -- (120,700.8) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (60,640.8) -- (140,640.8)(60,660.8) -- (140,660.8)(60,680.8) -- (140,680.8) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (60,620.8) -- (140,620.8) -- (140,700.8) -- (60,700.8) -- cycle ;
%Straight Lines [id:da11536840498544065] 
\draw [line width=1.5]    (120,660.8) -- (100,660.8) ;
%Straight Lines [id:da09443415166678082] 
\draw [line width=1.5]    (100,660.8) -- (80,680.8) ;
%Straight Lines [id:da8379640370273191] 
\draw [line width=1.5]    (120,660.8) -- (100,640.8) ;
%Straight Lines [id:da04028579824140888] 
\draw [line width=1.5]    (80,680.8) -- (100,640.8) ;
%Straight Lines [id:da9022422107770054] 
\draw [line width=1.5]    (100,660.8) -- (100,640.8) ;
%Straight Lines [id:da10686194521673875] 
\draw [line width=1.5]    (120,660.8) -- (80,680.8) ;
%Straight Lines [id:da716855825868624] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (60,640.8) -- (120,700.8) ;
%Straight Lines [id:da8186498055271281] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (60,640.8) -- (120,640.8) ;
%Straight Lines [id:da09024804133986408] 
\draw [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][line width=1.5]    (120,640.8) -- (120,700.8) ;

% Text Node
\draw (47,23) node [anchor=north west][inner sep=0.75pt]   [align=left] {1};
% Text Node
\draw (47,124) node [anchor=north west][inner sep=0.75pt]   [align=left] {2};
% Text Node
\draw (147,123) node [anchor=north west][inner sep=0.75pt]   [align=left] {3};
% Text Node
\draw (247,123) node [anchor=north west][inner sep=0.75pt]   [align=left] {4};
% Text Node
\draw (149,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {5};
% Text Node
\draw (347,224) node [anchor=north west][inner sep=0.75pt]   [align=left] {6};
% Text Node
\draw (47,323) node [anchor=north west][inner sep=0.75pt]   [align=left] {7};
% Text Node
\draw (148,323) node [anchor=north west][inner sep=0.75pt]   [align=left] {8};
% Text Node
\draw (347,323) node [anchor=north west][inner sep=0.75pt]   [align=left] {9};
% Text Node
\draw (442.5,323.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {10};
% Text Node
\draw (142,422) node [anchor=north west][inner sep=0.75pt]   [align=left] {11};
% Text Node
\draw (339,422) node [anchor=north west][inner sep=0.75pt]   [align=left] {12};
% Text Node
\draw (40,523) node [anchor=north west][inner sep=0.75pt]   [align=left] {13};
% Text Node
\draw (141.5,523.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {14};
% Text Node
\draw (242,523.3) node [anchor=north west][inner sep=0.75pt]   [align=left] {15};
% Text Node
\draw (42,623) node [anchor=north west][inner sep=0.75pt]   [align=left] {16};
\end{tikzpicture}

Following the method in \S\ref{hole}, we can list $A_h$ in the large $k$ limit for these reflexive cases:
\begin{enumerate}
    \item $\frac{3}{2}\log^2k-\frac{3}{2}\pi^2$,
    \item $2\log^2k-\frac{4}{3}\pi^2$, \inlineitem $2\log^2(k/2)-\frac{4}{3}\pi^2$, \inlineitem $2\log^2k-\frac{4}{3}\pi^2$,
    \item $\frac{5}{2}\log^2\left(\frac{A_1A_2A_3A_5}{A_4^3A_6^3}k\right)-\frac{7}{6}\pi^2$, \inlineitem $\frac{5}{2}\log^2\left(\frac{B_3B_4}{2B_1^3B_2B_5}k\right)-\frac{7}{6}\pi^2$,
    \item $2\log^2k-\pi^2$, \inlineitem $12\log^2k-\pi^2$, \inlineitem $12\log^2k-\pi^2$, \inlineitem $3\log^2k-\pi^2$,
    \item $\frac{7}{2}\log^2\left(\frac{E_5^2}{E_1^3E_2^2E_4}k\right)-\frac{5}{6}\pi^2$, \inlineitem $\frac{7}{2}\log^2\left(\frac{F_3^{1/2}F_4^{1/2}}{F_2}k\right)-\frac{5}{6}\pi^2$,
    \item $4\log^2k-\frac{2}{3}\pi^2$, \inlineitem $4\log^2\left(\frac{G_2G_3^{1/2}}{G_4^{3/2}}k\right)-\frac{2}{3}\pi^2$, \inlineitem $4\log^2k-\frac{2}{3}\pi^2$,
    \item $\frac{9}{2}\log^2k-\frac{1}{2}\pi^2$.
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% comment on F-maximization and Mahler measure
\rem{A possible way to explain this is via the $\cN=1$, $4d$ superconformal index. As an extension of the brane tilings paradigm, we can conjecture that the superconformal index, as the generalization of the Witten index, is given by the generating function of the dimer model \cite{Dijkgraaf:2007yr}. In particular, in the thermodynamic limit where the partition function of the dimer model is given by the Mahler measure, we can examine this conjecture. On the other side, for the superconformal index, which is defined as the partition function on $S^3\times S^1$, the thermodynamic limit is equivalent to taking the radius of the $S^1$ to zero. In this limit, the superconformal index reduces to the partition function of the $3d$ gauge theory on $S^3$ in which we have the $F$-theorem, \cite{Terashima:2012cx}. One interesting aspect is to prove the equivalence between the generating function of the dimer model and the superconformal index in general and beyond the thermodynamic limit.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A non-reflexive example for Seiberg duality
The discussions we have should hold in general, including non-reflexive polygons.
\begin{example}
The toric diagram for $Y^{3,0}$ has four vertices $(2,0),(2,-1),(-1,0),(-1,1)$ and two interior points $(1,0),(0,0)$. There are two toric phases which are \cite{Franco:2017jeo,Bao:2020kji}
\begin{equation}
    \includegraphics[width=4cm]{fig/Y30a.pdf},~~~~~~
    \includegraphics[width=4cm]{fig/Y30b.pdf}.
\end{equation}
Both of them yield the same Newton polynomial
\begin{equation}
    \frac{1}{2\sqrt{2}}z^2-\frac{1}{2\sqrt{2}}z^2w^{-1}-\frac{1}{2\sqrt{2}}z^{-1}w-\frac{1}{2\sqrt{2}}z^{-1}-\frac{3}{\sqrt{2}}z-\frac{3}{\sqrt{2}}=0,
\end{equation}
or equivalently,
\begin{equation}
    z^2-z^2w^{-1}-z^{-1}w-z^{-1}-6z+6=0.
\end{equation}
Hence, the duals have the same Mahler measure. In fact, for the second tiling, there are $4$ (out of $16$) bifundamentals have R-charge $1$. We again find that applying \eqref{isomahler} to the second tiling gives the correct Mahler measure. It is also worth noting that in this case, the second dimer degenerates to the first one (rather than some ``partially urban renewed'' dimer) with the four edges $e_{62,64}^{1,2}$ shrink to zero.
\end{example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Coefficients problem for specular duality and crystal melting
There are five such cases for reflexive polygons (No.5, 6, 9, 11, 14). Remarkably, they are exactly those special/exceptional cases in the discussion of specular duality. As labelled red in \eqref{specpairs}, No.5, 6, 9, 11 are the only reflexive polygons that cannot have the same Mahler measures as their specular duals no matter how we rescale/normalize the Newton polynomials. The self-dual No.14 is also exceptional as follows. In \eqref{specpairs}, the polygons in each row have the same number of boundary points (and hence same number of gauge nodes). We can see that they are all related by specular duality for different toric phases. However, No.14 is the only case that is not specular dual to any toric phases for other polygons in its row.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mahler flow for 16 reflexives:
\begin{example}
There are 16 reflexive Newton polygons. We plot the numerical results in Figure \ref{flownumerical}.
\begin{figure}[h]
    \centering
	\includegraphics[width=15cm]{fig/flow16.pdf}
	\caption{The Mahler flows for the 16 reflexive polygons with $k\geq k_\text{iso}$.}\label{flownumerical}
\end{figure}
\end{example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% F-theorem
\paragraph{The $F$-theorem} Before ending this subsection, let us take a look at $F$-maximization in 3d, which plays a similar role as $a$-maximization in 4d. It was discovered in \cite{Jafferis:2010un} that the R-symmetry for 3d $\mathcal{N}=2$ superconformal theory in the IR can be determined by considering the partition function on $S^3$:
\begin{equation}
    Z=\frac{1}{|\mathcal{W}|}\int_{\mathfrak{h}}\text{d}u\begin{bmatrix}\text{Contribution from}\\\text{vector multiplets}\end{bmatrix}\times\prod_i\det\nolimits_{\mathcal{R}_i}\text{e}^{l(1-R_i+iu)},
    \label{S3partition}
\end{equation}
where $|\mathcal{W}|$ is the order of the Weyl group of the gauge group and $\mathfrak{h}$ stands for the Cartan subalgebra. We are not spelling out the contribution from vector multiplets here (see \cite{Jafferis:2010un,Pufu:2016zxm} for more details). The chiral multiplet of R-charge $R_i$ transforms under the representation $\mathcal{R}_i$. The determinant in this rep with weights $\lambda_a^i$ is defined as
\begin{equation}
    \det\nolimits_{\mathcal{R}_i}f(u)\equiv\prod_{i=1}^{\dim\mathcal{R}_i}f\left(\sum_au_a\lambda_a^i\right).
\end{equation}
The function $l(x)$ in \eqref{S3partition}, from one-loop contribution from the chirals is
\begin{equation}
    l(x)=-\frac{i}{12}\pi^2+\frac{i}{2}x^2-x\log(1-\text{e}^{2ix})+\frac{i}{2}\text{Li}_2(\text{e}^{2ix}).
\end{equation}
As one may check, this is exactly the same as $-\pi m_\text{iso}$ appearing in \eqref{isomahler} with a single variable, viz,
\begin{equation}
    l(x)=-x\log(2\sin(x))-\Lambda(x).
\end{equation}
Indeed, the derivative of $l(x)$ is $l'(x)=-\pi x\cot(x)$ \footnote{This was also observed in \cite{Yamazaki:2012cp}.}. Therefore, it is natural to expect that there might be some relations between $F$-maximizations and the Mahler measure.

It is still not clear how the two concepts are connected, but one might be able to find clues in some simplest examples. Consider the Wess-Zumino model with an O$(N)$-invariant superpotential $W=g\Phi_0\sum\limits_{i=1}^N\Phi_i^2$, where $\Phi_{0,\dots,N}$ are chiral multiplets. The free energy is
\begin{equation}
    F=\log Z=-Nl(1-R)-l(2R-1),
\end{equation}
where $R_0=2-2R$ and $R_{1,\dots,N}=R$ \cite{Giombi:2014xxa}. As we can see, $F$-maximization in this case is exactly the same as the maximization of the isoradial Mahler measure
\begin{equation}
    m_\text{iso}=N\left(\frac{\pi-\theta}{\pi}\log(2\sin(\pi-\theta))+\frac{1}{\pi}\Lambda(\pi-\theta)\right)+\frac{2\theta-\pi}{\pi}\log(2\sin(2\theta-\pi))+\frac{1}{\pi}\Lambda(2\theta-\pi).
\end{equation}
For instance, when $N=2$, which is also known as the $XYZ$ model, $m_\text{iso}$ turns out to be the same as the one for the dimer with one hexagon as the fundamental domain. There are four rhombus angles of $(\pi-\theta)$ and two of $(2\theta-\pi)$. Then $m_\text{iso}$ and $F$ are maximized at $\theta=\pi/3$ (or equivalently, $R=2/3$), and the R-charges for $\Phi_{0,1,2}$ are all $2/3$.

It is well-known that the SQED with a pair of conjugate chirals $Q,\Tilde{Q}$ and no Chern-Simons (CS) interaction is dual to the $XYZ$ model \cite{Aharony:1997bx}. Its free energy is
\begin{equation}
    F=-2l(r)-l(1-2r),
\end{equation}
where we only have one parameter $r$ since the R-symmetry can only mix with the U(1) flavour symmetry. Again, maximizing $F$ concides with maximizing certain $m_\text{iso}$. In this case, they reach the maximum when $r=1/3$. In the $XYZ$ model, $X=\Phi_0$ is dual to the meson $Q\Tilde{Q}$ with R-charge $2-2R=2r=2/3$ while $Y,Z=\Phi_1\pm i\Phi_2$ are dual to the monopole operators with R-charge $R=1-r=2/3$.

More generally, if we consider $U(N)$ flavour symmetry and CS level $k$, the partition function is \cite{Jafferis:2010un,Klebanov:2011td}
\begin{equation}
    Z=\int_{-\infty}^{+\infty}\text{d}u\text{e}^{i\pi ku^2}\text{e}^{N(l(1-r+iu)+l(1-r-iu))}.
\end{equation}
In the large $N$ limit while keeping $\frac{2k}{\pi N}$ fixed, the free energy can be expanded as
\begin{equation}
    F=-2Nl(1-r)+o(\log N).
\end{equation}
Therefore, at leading order, we have the Mahler measure
\begin{equation}
    m_\text{iso}=2N\left(\frac{\pi-\theta}{\pi}\log(2\sin(\pi-\theta))+\frac{1}{\pi}\Lambda(\pi-\theta)\right).
\end{equation}
This is maximized at $\theta=\pi/2$. In other words, $r=1/2+\mathcal{O}(1/N)$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% isoradial Ronkin function
Ronkin functions, on the other hand, are more difficult to be so simply expressed, even for the isoradial case. Following \cite{Kenyon:2003uj}, the Mahler measure (either isoradial or non-isoradial) appears in computing the partition function $Z$ (per fundamental domain) of the (infinite) dimer $\mathcal{G}$:
\begin{equation}
\begin{split}
    m(P)=\log Z=&\lim_{n\rightarrow\infty}\frac{1}{n^2}\log\left(\right.(-\det(K_n(1,1))+\det(K_n(-1,1))\\
    &+\det(K_n(1,-1))+\det(K_n(-1,-1)))/2\left.\right),
\end{split}
\end{equation}
where $K_n(z,w)$ is the Kasteleyn matrix for the dimer $\mathcal{G}_n$. For Ronkin functions, one can simply replace $z$ and $w$ by $\text{e}^xz$ and $\text{e}^yw$. Hence, we have $K_n(\pm\text{e}^x,\pm\text{e}^y)$ in the determinants. This change makes the method in \cite{de2007partition} even more non-trivial when applied to Ronkin functions. Nevertheless, inspired by the derivation for isoradial Mahler measure, we can take the derivative of Ronkin function with respect to $\theta_I$. For simplicity, we shall restrict to the cases when $k_\text{iso}=k_0\equiv\max\limits_{|z|=|w|=1}(|p|)$ (while things would be more complicated when $k_\text{iso}<k_0$). Thus,
\begin{equation}
\begin{split}
    \frac{\partial R(x,y)}{\partial\theta_I}&=\frac{1}{(2\pi i)^2}\int_{|z|=\text{e}^x,|w|=\text{e}^y}\frac{\partial\log P(z,w)}{\partial\theta_I}\frac{\text{d}z}{z}\frac{\text{d}w}{w}
    =\frac{1}{(2\pi i)^2}\int_{|z|=\text{e}^x,|w|=\text{e}^y}\frac{\partial P/\partial\theta_I}{P}\frac{\text{d}z}{z}\frac{\text{d}w}{w},
\end{split}
\end{equation}
where only terms containing $2\sin(\theta_I)$ would survive in $\partial P/\partial\theta_I$:
\begin{equation}
    P'\equiv\frac{\partial P}{\partial\theta_I}=\sum_{(m,n)}2\cos(\theta_I)\left(\prod_{J\neq I}2\sin(\theta_J)\right)z^mw^n.
\end{equation}
Since $P$ is a Laurent polynomial, using residue theorem, we have
\begin{equation}
    \frac{\partial R(x,y)}{\partial\theta_I}=\sum_j\text{Res}\left(\sum_i\text{Res}\left(\frac{P'}{zwP},a_i\right),b_j\right),
\end{equation}
where $a_i$ and $b_j$ are poles of $zwP(z,w)$ in the interior of $\{|z|=\text{e}^x\}$ and $\{|w|=\text{e}^y\}$ respectively. To be precise, these should be poles of $zw\Tilde{P}(z,w)$ where $\Tilde{P}=z^mw^nP$ such that $\Tilde{P}$ only has non-negative powers of $z$ and $w$ (and hence no negative powers in $\Tilde{P}'$ in the numerator). This would not change the result since we are multiplying both the numerator and the denominator by $z^mw^n$ in $\frac{P'}{zwP}$.

Now we can in principle integrate over $\theta_I$ to obtain $R(x,y)$. To determine the constant of integration, let us continuously deform the dimer model such that all the rhombus angles tend to either 0 or $\pi/2$. This is always plausible according to \cite{Kenyon_2002}. Suppose the rhombus angles $\phi_I$ go to 0 and the remaining rhombus angles $\psi_J$ go to $\pi/2$, then
\begin{equation}
    R(x,y)=\sum_I\int_0^{\phi_I}\frac{\partial R}{\partial\theta_I}\text{d}\theta_I+\sum_J\int_{\pi/2}^{\psi_J}\frac{\partial R}{\partial\theta_J}\text{d}\theta_J+R_{(0,\dots,0,\pi/2,\dots,\pi/2)}.\label{isoronkin}
\end{equation}
For the deformed dimer, we have a chain with alternating black and white nodes along the edges of weight 2 corresponding to rhombus angles $\pi/2$ (while rhombus angles 0 give 0 weights). Therefore, the Ronkin function now degenerates to a univariate function, say $R(y)$. As $\frac{1}{2\pi i}\int_{|z|=\text{e}^x}\frac{\text{d}z}{z}=1$, we have
\begin{equation}
\begin{split}
    R_{(0,\dots,0,\pi/2,\dots,\pi/2)}=R(y)&=\frac{1}{2\pi i}\int_{|w|=\text{e}^y}\frac{\log P(w)}{w}\text{d}w\\
    &=\frac{1}{2\pi i}\int_{|w|=1}\frac{\log P(\text{e}^yw)}{w}\text{d}w
    :=\frac{1}{2\pi i}\int_{|w|=1}\frac{\log Q_y(w)}{w}\text{d}w,
\end{split}
\end{equation}
where $Q_y(w)$ is the same as $P(\text{e}^yw)$, but we emphasize that the factors containing $y$ are treated as parts of the coefficients. As the Mahler measure is invariant under GL$(2,\mathbb{Z})$ transformations, we can write $Q_y=a_0(w-a_1)\dots(w-a_n)$ (where $a_i$ implicitly depends on $y$) and apply Jensen's formula:
\begin{equation}
    R_{(0,\dots,0,\pi/2,\dots\pi/2)}=\log|a_0|+\sum_{i=1}^n\max\{0,\log|a_i|\}.
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
